Adaptive CSMA under the SINR Model: Efficient Approximation Algorithms for Throughput and Utility Maximization

We consider a Carrier Sense Multiple Access (CSMA) based scheduling algorithm for a single-hop wireless network under a realistic Signal-to-interference-plus-noise ratio (SINR) model for the interference. We propose two local optimization based approximation algorithms to efficiently estimate certain attempt rate parameters of CSMA called fugacities. It is known that adaptive CSMA can achieve throughput optimality by sampling feasible schedules from a Gibbs distribution, with appropriate fugacities. Unfortunately, obtaining these optimal fugacities is an NP-hard problem. Further, the existing adaptive CSMA algorithms use a stochastic gradient descent based method, which usually entails an impractically slow (exponential in the size of the network) convergence to the optimal fugacities. To address this issue, we first propose an algorithm to estimate the fugacities, that can support a given set of desired service rates. The convergence rate and the complexity of this algorithm are independent of the network size, and depend only on the neighborhood size of a link. Further, we show that the proposed algorithm corresponds exactly to performing the well-known Bethe approximation to the underlying Gibbs distribution. Then, we propose another local algorithm to estimate the optimal fugacities under a utility maximization framework, and characterize its accuracy. Numerical results indicate that the proposed methods have a good degree of accuracy, and achieve extremely fast convergence to near-optimal fugacities, and often outperform the convergence rate of the stochastic gradient descent by a few orders of magnitude.

==> ArXiv Version TON/abstract.tex <==
We consider a Carrier Sense Multiple Access (CSMA) based scheduling algorithm for a single-hop wireless network under a realistic Signal-to-interference-plus-noise ratio (SINR) model for the interference. We propose two local optimization based approximation algorithms to efficiently estimate certain attempt rate parameters of CSMA called fugacities. It is known that adaptive CSMA can achieve throughput optimality by sampling feasible schedules from a Gibbs distribution, with appropriate fugacities. Unfortunately, obtaining these optimal fugacities is an NP-hard problem. Further, the existing adaptive CSMA algorithms use a stochastic gradient descent based method, which usually entails an impractically slow  (exponential in the size of the network) convergence to the optimal fugacities. To address this issue, we first propose an algorithm to estimate the fugacities, that can support a given set of desired service rates. The convergence rate and the complexity of this algorithm are independent of the network size, and depend only on the neighborhood size of a link. Further, we show that the proposed algorithm corresponds exactly to performing the well-known Bethe approximation to the underlying Gibbs distribution. Then, we propose another local algorithm to estimate the optimal fugacities under a utility maximization framework, and characterize its accuracy. Numerical results indicate that the proposed methods have a good degree of accuracy, and achieve extremely fast convergence to near-optimal fugacities, and often outperform the convergence rate of the stochastic gradient descent by a few orders of magnitude.
 
 


%We consider a CSMA based scheduling algorithm for a single-hop wireless network under a realistic SINR (signal-to-interference-plus-noise ratio) model for the interference. We propose local optimization based algorithms to efficiently estimate certain attempt rate parameters of the algorithm called fugacities. It is known that adaptive CSMA based algorithms can achieve throughput optimality, by sampling feasible schedules from a Gibbs distribution, with appropriate fugacities. Unfortunately, obtaining the optimal fugacities for a desired service rate vector is an NP-hard problem. Further, the existing adaptive CSMA algorithms use a stochastic gradient descent based method, which usually entails an impractically slow  (exponential in the size of the network) convergence to the optimal fugacities. In contrast, the convergence rate and the complexity of the algorithms we propose are independent of the network size, and depend only on the neighborhood size of a link. Further, we show that the proposed algorithm corresponds exactly to performing the well-known Bethe approximation to the underlying Gibbs distribution. We also propose an algorithm for a related problem of computing the optimal fugacities under a utility maximization framework.  Numerical results indicate that the proposed methods achieve extremely fast convergence to near-optimal fugacities, and often outperform the convergence rate of the stochastic gradient descent by a few orders of magnitude.

\begin{comment}
In this paper, we consider an adaptive CSMA based scheduling algorithm for a single-hop wireless network under a realistic SINR (signal-to-interference-plus-noise ratio) model for the interference, and propose an order-optimal algorithm to estimate certain parameters of the algorithm called fugacities. Recent work has shown that adaptive CSMA based algorithms can achieve throughput optimality, by sampling feasible schedules from a product form Gibbs distribution. In order to support a desired service rate vector using adaptive CSMA,  certain parameters of the Gibbs distribution, called fugacities, must be estimated. Unfortunately, estimating the optimal fugacities for a desired service rate vector is an NP-hard problem. Further, the existing adaptive CSMA algorithms use a stochastic gradient descent based method, which usually entails an impractically slow convergence to the optimal fugacities. We propose an efficient and scalable approximation based on a local Gibbs optimization technique to estimate the fugacities corresponding to the desired service rates. We show that the proposed local Gibbs optimization corresponds exactly to performing the well-known Bethe approximation to the global Gibbs optimization. We also consider two special cases of the SINR interference model, and derive clsoed form expressions for the fugacities. Numerical results indicate that the proposed method achieves an almost instantaneous convergence to near-optimal fugacities, and often outperforms the convergence rate of the stochastic gradient descent by a few orders of magnitude. Notably, the proposed method is also quite robust to gradual changes in the desired service rates, as well as to changes in the topology. 
\end{comment}



==> ArXiv Version TON/conclusions.tex <==
We considered the adaptive CSMA algorithm under the SINR interference model, which is known to be throughput optimal. Under this model, we first proposed a distributed algorithm, namely the local Gibbsian method to efficiently estimate the fugacities, for a given service rate requirements. The convergence rate and the complexity of the proposed algorithm depend only on the maximum size of a link's neighbourhood. We proved that our approximation corresponds exactly to performing the well known Bethe approximation to the global Gibbsian problem. We also proposed an approximation algorithm to estimate the fugacities under a utility maximization framework. Our numerical results indicate that the proposed approximation algorithms can lead to a good degree of accuracy, and improve the convergence time by a few orders of magnitude, compared to the existing stochastic gradient descent methods. 

\section*{Acknowledgement}
 The authors express their sincere gratitude to Dr. Pascal Vontobel for his valuable comments on this work.

==> ArXiv Version TON/gibbs_bethe.tex <==
We first prove certain important structural properties of the BFE, which we then use to establish an equivalence between the local Gibbsian method (Algorithm 1) and the Bethe approximation. In particular, the above equivalence hinges on establishing the following two important properties, which are formalized subsequently in Lemmas \ref{lemma_max_entropy} through \ref{lemma_fug}.
\begin{itemize}
\item At a stationary point of the BFE, the relation between the factor and the variable marginals is captured by the local Gibbsian problem.
%\item The local Gibbsian problem characterizes the relation between the factor and variable marginals at a stationary point of the BFE.
\item The factor and variable marginals corresponding to a stationary point of the BFE uniquely determine the fugacities.
\end{itemize}
\noindent \emph{Remark:} The above properties are derived for the Bethe approximation under the SINR model considered in this paper. The Bethe approximation under general settings may not satisfy these properties.
\subsection{Characterization of the stationary points of the BFE}
In this subsection, we characterize the stationary points of the Bethe free energy $F_B(\bn,\bv)$ \eqref{eq_bfe} in Lemmas \ref{lemma_max_entropy} and \ref{lemma_fug}.
The following Lemma asserts that the stationary points of $F_B(\bn,\bv)$ satisfy a maximum entropy property.
\begin{lemma} \label{lemma_max_entropy}
 Let $F_B(\bn,\bv)$ \eqref{eq_bfe} denote the BFE corresponding to the fugacities $\{\lambda_i\}_{i=1}^N$. Let $(\bn^*, \bv^*)$ be a stationary point of $F_B(\bn,\bv)$ that satisfies the feasibility constraints in \eqref{eq_bethe_min}, \eqref{eq_bn_feasible}. Then, for each $i\in \N$, the factor marginal $\b_i^*$ is related to its corresponding variable marginals $\{b_j^*\}_{j \in \N_i}$, through the following constrained entropy maximization problem, parametrized by the variable marginals $\{b_j^*\}_{j \in \N_i}$:
 \begin{align}
&\b_i^*=\arg \max\limits_{\b_i} \H_i(\b_i), \text{     subject to} \label{opt_local_entropy}\\
&\b_i(\x^{(i)}) \geq 0, \; \forall \x^{(i)} \in \I_i; \sum_{\x^{(i)} \in \I_i} \b_i(\x^{(i)})=1,\nonumber\\
 &\sum\limits_{\x^{(i)} \setminus \{x_j \}} \b_i(\x^{(i)})= b_j^*(x_j), \hspace{0.2cm}  \; \forall j \in \N_i,\; x_j =1. \label{eq_dual}
\end{align}
 \end{lemma}
\begin{proof}
Proof is provided in Appendix~\ref{proof_max_entropy}.
\end{proof}
Further, it can be shown \cite[Section 3.5]{libin_book} that there is a unique solution to the maximum entropy problem \eqref{opt_local_entropy}. Specifically, the variable marginals $\{b_j^*\}_{j \in \N_i}$ uniquely characterize the corresponding factor marginal $\b_i^*$, through the local Gibbsian problem \eqref{opt_local_alternate}; this is formalized in Lemma \ref{lemma_libin}.
%\begin{comment}
%derived by considering the dual problem of \eqref{opt_local_entropy}. It can also be proved that the distribution $\bn^*$ defined in \eqref{eq_thm2}, has the maximal entropy property, because of its product form, as shown in Lemma \ref{lemma_libin}.
%\end{comment}

 \begin{lemma} \label{lemma_libin}
Consider the following local Gibbsian problem defined by the variable marginals $\{b_j^*\}_{j \in \N_i}$:
\begin{align}
v_i = \arg\max\limits_{r \in \R^{\N_i}} \sum\limits_{k \in \N_i} b_k^*(1) r_{k} - \ln \Big(\sum\limits_{y \in \I_i} \exp\Big(\sum\limits_{k \in \N_i} y_k r_{k} \Big)\Big). \label{opt_local_alternate}
\end{align} 
%where $F(r):=\sum\limits_{k \in \N_i} b_k^*(1) r_{k} - \ln \Big(\sum\limits_{y \in \I_i} \exp\Big(\sum\limits_{k \in \N_i} y_k r_{k} \Big)\Big).$
Then the corresponding factor marginal (optimal solution of \eqref{opt_local_entropy}) is given by
\begin{align}
\b_i^*(\x^{(i)})& = \frac{1}{Z_i} \exp\Big(\sum\limits_{k \in \N_i} x_k v_{ik} \Big), & \forall \x^{(i)} \in \I_i, \label{eq_opt_factor_marg}
\end{align}
where $v_i=[v_{ik}]_{k \in \N_i}$ is the solution of \eqref{opt_local_alternate}, $Z_i$ is a normalization constant.
%\begin{align*}
%F(r):=\sum\limits_{k \in \N_j} b_k^*(1) r_{k} - \ln \Big(\sum\limits_{y \in \I_j} \exp\Big(\sum\limits_{k \in \N_j} y_k r_{k} \Big)\Big).
%\end{align*} 
 \end{lemma}
\begin{proof}
Proof follows by considering the dual problem of \eqref{opt_local_entropy}. The proof can be found in  \cite[Section 3.5]{libin_book}.
\end{proof}

{Next, in Lemma \ref{lemma_fug}, we prove that the factor and variable marginals at a stationary point of the BFE uniquely characterize the fugacities.}
\begin{lemma} \label{lemma_fug}
Let $F_B(\bn,\bv)$ \eqref{eq_bfe} denote the BFE corresponding to the fugacities $\{\lambda_i\}_{i=1}^N$. Let $(\bn^*, \bv^*)$ be a stationary point of the $F_B(\bn,\bv)$. Then the fugacities are uniquely determined by the factor and variables marginals $(\bn^*, \bv^*)$ as follows:
\begin{align}
\lambda_i&= \left(\frac{1-b^*_i(1)}{b_i^*(1)}\right)^{d_i-1}\prod\limits_{j \in \ni} e^{v_{ji}}, \; \; \forall i \in \N, \label{eq_lf_gf}
\end{align}
where $v_{ji}$ is an element of the vector $v_j=[v_{jk}]_{k \in \N_j}$, that characterizes the factor marginal $\b_j^*$ of some $j\in \N_i$.
\end{lemma}
\begin{proof}
Proof is provided in Appendix \ref{proof_fugacities}.
\end{proof}
In Lemmas \ref{lemma_max_entropy}, \ref{lemma_fug} we have derived the necessary conditions that a stationary point of the BFE should satisfy. In Appendix \ref{proof_complete}, we show that the conditions in these two Lemmas together constitute a sufficient condition for a stationary point of the BFE.
\subsection{Local Gibbsian method gives the Bethe approximated fugacities}
We are now in a position to state a key result of this paper, which asserts that the approximated global fugacities \eqref{eq_lf_gf0} obtained by solving the local Gibbsian problems \eqref{opt_local_alternate0} correspond exactly to the Bethe approximated fugacities. We formalize this result through Definition \ref{def_bethe_fug}, Theorem \ref{thm_bethe_main}.
 
\begin{definition} (Bethe approximated fugacities) \label{def_bethe_fug}
For a given set of service rates $\{s_i\}_{i=1}^N$, a set of fugacities $\{\lambda_i\}_{i=1}^N$ are said to be Bethe approximated fugacities if the following holds:
``Consider the BFE $F_B(\bn,\bv)$ corresponding to the fugacities $\{\lambda_i\}_{i=1}^N$. Then there should exist a stationary point $(\bn^*,\bv^*)$ point of the BFE such that the corresponding variable marginals are equal to the given service rates, \ie, $b_i^*(1)=s_i, \forall i$".
\end{definition}
\begin{theorem} \label{thm_bethe_main} 
Let $\{s_i\}_{i=1}^N$ be the desired service rates.
\begin{itemize} 
\item[1.]  Then the global fugacities $\{\lt_i\}_{i=1}^N$ estimated in \eqref{eq_lf_gf0} are the Bethe approximated fugacities for $\{s_i\}_{i=1}^N$. 
\item[2.] For a given set of service rates, the Bethe approximated fugacities are unique. 
\end{itemize}
\end{theorem}

\begin{proof}
Consider the BFE \eqref{eq_bfe_new} corresponding to the fugacities $\{\lt_i\}_{i=1}^N$. We show there exists a stationary point $(\{\underline{\b}_j\}, \{\underline{b}_j\})$ of the BFE, given by \eqref{eq_thm1}-\eqref{eq_thm2}, such that the corresponding variable marginals $\{\underline{b}_j(1)\}$ \eqref{eq_thm1} are equal to the desired service rates $\{s_i\}_{i=1}^N$.
%Then there is a stationary point $(\{\underline{\b}_j\}, \{\underline{b}_j\})$  of the BFE, given by \eqref{eq_thm1}-\eqref{eq_thm2}. In particular, the variable marginals $\{\underline{b}_j(1)\}$ \eqref{eq_thm1} corresponding to the stationary point are equal to the desired service rates.
%the variable marginals are equal to the desired service rates at the following stationary point given in $(\{\underline{\b}_j\}, \{\underline{b}_j\})$ in \eqref{eq_thm1}-\eqref{eq_thm2}".
%of marginals $(\{\underline{\b}_j\}, \{\underline{b}_j\})$ in \eqref{eq_thm1}-\eqref{eq_thm2} is a stationary point of the BFE \eqref{eq_bfe_new}".
\begin{align}
F_B(\bn,\bv)&= \sum\limits_{i=1}^N   -b_i(1) \ln\lt_i  - \H_i(\b_i)  +  (d_i-1) H_i(b_i), \label{eq_bfe_new} \\
\underline{b}_j(1)&=s_j, \; \underline{b}_j(0)=1-s_j, \; \; \forall j, \label{eq_thm1}\\
 \underline{\b}_j(\x^{(j)})& = \frac{1}{Z_j} \exp\Big(\sum\limits_{k \in \N_j} x_k \lf_{jk} \Big), \; \; \forall \x^{(j)} \in \I_j, \; \forall j, \label{eq_thm2}
\end{align}
where $\lf_j=[\lf_{jk}]_{k \in \N_j}$ is the local fugacity vector at link $j$ obtained from \eqref{opt_local_alternate0}, and $Z_j$ is the corresponding normalization constant. 

Now we use the structural properties of the BFE derived in Lemmas 2 through 4 to complete the proof. In particular, recall from \eqref{opt_local_alternate0} that the local fugacity vector $\lf_j=[\lf_{jk}]_{k \in \N_j}$ is obtained by solving the local Gibbsian problem \eqref{opt_local_alternate0}, which is same as \eqref{opt_local_alternate}. Hence, due to Lemma \ref{lemma_libin}, it is clear that the set of marginals $(\{\underline{\b}_j\}, \{\underline{b}_j\})$ in \eqref{eq_thm1}-\eqref{eq_thm2} satisfy the maximum entropy property stated in Lemma \ref{lemma_max_entropy}. 

Next, due to the definition \eqref{eq_lf_gf0} of the global fugacities $\{\lt_i\}_{i=1}^N$, the variable and factor marginals defined in \eqref{eq_thm1}-\eqref{eq_thm2} immediately satisfy the condition \eqref{eq_lf_gf} in Lemma \ref{lemma_fug}. 

Therefore, $(\{\underline{\b}_j\}, \{\underline{b}_j\})$ given in \eqref{eq_thm1}-\eqref{eq_thm2} is a stationary point of the BFE \eqref{eq_bfe_new}. Further, note that the corresponding variable marginals $\{\underline{b}_j(1)\}$ \eqref{eq_thm1} at this stationary point are equal to the desired service rates $\{s_i\}_{i=1}^N$. Hence, the fugacities $\{\lt_i\}_{i=1}^N$ are the Bethe approximated fugacities  for $\{s_i\}_{i=1}^N$.

Next, we prove the uniqueness of the Bethe approximated fugacities. For the given service rates $\{s_i\}_{i=1}^N$, let us assume that two sets of fugacities $\{\lambda_i^1\}_{i=1}^N$, $\{\lambda_i^2\}_{i=1}^N$ satisfy the definition of the Bethe approximated fugacities. Let $F_B^1(\bn,\bv)$, $F_B^2(\bn,\bv)$ be the BFE functions corresponding to the  fugacities $\{\lambda_i^1\}_{i=1}^N$, $\{\lambda_i^2\}_{i=1}^N$ respectively. Then there should exist stationary points $(\{\b_j^1\},\{b_j^1\} )$, $(\{\b_j^2\},\{b_j^2\} )$ of their corresponding BFE functions such that the variables marginals are equal to the service rates, \ie, $\{b_j^1(1)\}=\{b_j^2(1)\}=\{s_j\}$. Since the variable marginals are same, due to Lemmas \ref{lemma_max_entropy}, \ref{lemma_libin}, the factor marginals corresponding to these stationary points should be the same. In other words,  \ie,  $(\{\b_j^1\},\{b_j^1\} )= (\{\b_j^2\},\{b_j^2\} )$. Then \eqref{eq_lf_gf} from Lemma \ref{lemma_fug} asserts that $\{\lambda_i^1\}_{i=1}^N = \{\lambda_i^2\}_{i=1}^N$. Hence, for a given set of service rates, the Bethe approximated fugacities are unique.
\end{proof}

%Next, we state a corollary which asserts the uniqueness of the Bethe approximated fugacities for a given service rates.

%\begin{cor}
%For a given service rate requirements, the Bethe approximated fugacities are unique. 
%\end{cor}
%\begin{proof}
%For the given service rates $\{s_i\}_{i=1}^N$, let us assume that two sets of fugacities $\{\lambda_i^1\}_{i=1}^N$, $\{\lambda_i^2\}_{i=1}^N$ satisfy the definition of the Bethe approximated fugacities. Let $F_B^1(\bn,\bv)$, $F_B^2(\bn,\bv)$ be the BFE functions corresponding to the  fugacities $\{\lambda_i^1\}_{i=1}^N$, $\{\lambda_i^2\}_{i=1}^N$ respectively. Then there should exist stationary points $(\{\b_j^1\},\{b_j^1\} )$, $(\{\b_j^2\},\{b_j^2\} )$ of their corresponding BFE functions such that the variables marginals are equal to the service rates, \ie, $\{b_j^1(1)\}=\{b_j^2(1)\}=\{s_j\}$. Since the variable marginals are same, due to Lemma \ref{lemma_max_entropy}, \ref{lemma_libin} the factor marginals corresponding to these stationary points should be the same. In other words,  \ie,  $(\{\b_j^1\},\{b_j^1\} )= (\{\b_j^2\},\{b_j^2\} )$. Then \eqref{eq_lf_gf} from Lemma \ref{lemma_fug} asserts that $\{\lambda_i^1\}_{i=1}^N = \{\lambda_i^2\}_{i=1}^N$. Hence, for a given service rate requirements, the Bethe approximated fugacities are unique.
%Let $\{s_i\}_{i=1}^N$ be the desired service rates. Let us assume there are two sets of fugacities $\{\lambda_i^1\}_{i=1}^N$, $\{\lambda_i^2\}_{i=1}^N$ which satisfy the definition of the Bethe approximated fugacities. 
%To prove this, we have to show that there is a unique set of fugacities for which their corresponding BFE will have the service rates as its variable marginals at a stationary point. This can be deduced as follows: a) If the variable marginals at the stationary point are set to the service rates as shown in \eqref{eq_thm1},  then the factor marginals at that stationary point are uniquely determined due to Lemma \ref{lemma_libin}. b) Further, the fugacities are uniquely determined from these factor and variable marginals due to Lemma \ref{lemma_fug}. Hence, there is one to one mapping from the service rates to the Bethe approximated fugacites.
%\end{proof}

%Further, the uniqueness of the fugacities follows from \eqref{eq_lf_gf} which states that the fugacities are uniqu
%Let us assume that there exist some other fugacities $\{\lambda^{'}_i\}_{i=1}^N$ such that their corresponding BFE will have the service rates as its variable marginals at a stationary point. 
%Further, the uniqueness of the fugacities follows from the fact that the maximum entropy problem \eqref{opt_local_entropy} has a unique solution. This concludes the proof of Theorem \ref{thm_bethe_main}. 

% \emph{Remark on throughput optimality}: Although the Bethe approximated fugacities obtained using \eqref{eq_lf_gf0}, correspond closely to the desired service rates in many practical scenarios, the fugacities are still approximate. In particular, a CSMA algorithm which uses these approximate fugacities is not technically throughput optimal. In order to obtain a provably throughput optimal CSMA algorithm, one can simply use the Bethe approximated fugacities as a very good initial iterate for the usual stochastic gradient descent.



%Using Lemma \ref{lemma_max_entropy},  the optimal factor marginals $\{\b_j, j \in \N\}$ can be obtained, if each link $j \in \N$ independently  solves the following maximum entropy optimization problem over the valid distribution on $\{0,1\}^{|\N_j|}$:





%\end{lemma}
%\begin{proof}
%The proof folo
%\end{proof}
%
%
%Moreover, the vector $v_j$ can be obtained as solution to 
%\begin{align}
%v_{j} = \arg\max\limits_{r \in \R^{\N_j}} F(r), \label{opt_local_alternate}
%\end{align} 
%where, the function $F: \R^{\N_j} \rightarrow \R$ is defined by,
%\begin{align*}
%F(r):=\sum\limits_{k \in \N_j} s_k r_{k} - \ln \left(\sum\limits_{y \in \I_j} \exp\left(\sum\limits_{k \in \N_j} y_k r_{k} \right)\right).
%\end{align*} 


%
%\emph{Remark on throughput optimality:} The estimates of the fugacities obtained through our algorithm closely correspond to the desired service rates and often outperform the accuracy of the stochastic gradient descent based algorithms in most practical time scales as evidenced through our numerical results. However, the fugacities are still only approximate. In other words, the CSMA algorithm which uses the approximated global fugacities from \eqref{eq_lf_gf} is not technically throughput-optimal. In order to obtain a provably throughput optimal adaptive CSMA algorithm, we can use the approximate global fugacities as a good initial iterate for the stochastic gradient descent on the global Gibbsian problem. 


==> ArXiv Version TON/intro_1.tex <==

The problem of link scheduling for maximum throughput has been widely studied, particularly with emphasis on the maximum-weight scheduling framework, developed in \cite{tassiulas,TE93}. In spite of its throughput maximizing property, maximum-weight scheduling requires centralized control, and necessitates the solution of an NP-hard problem for each scheduling decision. Several works have attempted to modify the maximum-weight algorithm, so as to make it more amenable to simple, distributed implementation \cite{chaporkar2008throughput,dimakis2006sufficient,wu06}. However, these greedy algorithms do not achieve full throughput.


In a series of recent papers \cite{libin,dshah,qcsma}, a class of distributed link scheduling algorithms called adaptive CSMA algorithms have been proposed and proven to be throughput optimal, \ie, they can support any achievable service rate vector. The central idea behind these algorithms lies in using a reversible Markov chain to sample feasible schedules from a product form distribution called the Gibbs distribution \cite[Chapter 7]{bremaud}. Specifically, each link adaptively adjusts its transmission attempt rate (also known as its fugacity) in order to ensure sufficient average service rate. 

In order to support a given feasible service rate vector using CSMA, the corresponding fugacities have to be computed. Unfortunately, determining the appropriate fugacities corresponding to the desired service rates is an NP-hard problem \cite{libin}. In \cite{libin}, the optimal fugacities are computed as a solution to an optimization problem (here after referred to as the Gibbsian problem), using a stochastic gradient descent algorithm. Each iteration of the gradient descent requires estimating the average service rates under the current iterate of the fugacities, which in turn entails waiting for the underlying Markov chain to reach steady-state. This `mixing time' of the underlying Markov chain could be very large (exponential in the size of the network), depending on the network load and topology \cite{hardness}, \cite{fast_mixing}. Therefore, the existing adaptive CSMA algorithms \cite{libin} do not provide a practical way to estimate the fugacities, although they effectively support the desired service rates once the optimal fugacities are estimated \cite{parallel_chains}. The main focus of this paper is in proposing efficient methods to estimate the fugacities, under a realistic SINR (signal-to-interference-plus-noise ratio) model for the interference. Specifically, we consider the following two scenarios under which fugacities are to be computed:
\begin{itemize}
\item The service rate requirements of the links are known. The objective is to support these average service rates.
\item The service rate requirements are not known, but each link has a utility function of its average service rate. The objective is to maximize the sum utility of the network.
\end{itemize}

 A simple conflict graph based interference model ~\cite{libin, dshah, qcsma}  is widely used in the wireless context due to its simplicity and tractability, although it does not adequately capture the complex nature of the wireless interference \cite{graph_limitations}. More specifically, a {conflict graph} based interference model ignores the fact that whether or not two links can transmit simultaneously, depends on the transmission state of the other links and their spatial locations. Some recent papers extend the adaptive CSMA framework to a more realistic interference models like the SINR model \cite{sinr_mimo, sinr_mimo_journal}, and Rayleigh faded channels \cite{ncc_paper}. However, these papers also essentially employ stochastic gradient descent on a Gibbsian function to estimate the fugacities, and hence suffer from impractically slow convergence rates. 
 
For the conflict graph based interference model assumed in \cite{libin}, approximate but efficient methods to compute the fugacities have been proposed \cite{bp_csma,bethe_jshin} using a popular variational technique called the Bethe approximation \cite{yedidia}. However, the solutions given in \cite{bp_csma,bethe_jshin}, cannot be directly extended to SINR based interference model. This is because the conflict graph based interference model corresponds to a simple pair-wise interaction model \cite {yedidia}, while the SINR model involves higher order interactions. The presence of these higher order interactions makes the extension non-trivial. Even for graphical models with higher order interactions, there are well known algorithms like Belief propagation (BP) \cite{yedidia} for solving the Bethe approximation problem. However, in the context of adaptive CSMA under the SINR model, they can directly be used only to estimate the service rates given the fugacities, but not the other way around. 

%One way to circumvent this limitation, and use an algorithm like BP for finding the fugacities, is to use the estimates of the service rates computed using BP, as a replacement for the underlying Markov chain based estimates, in each iteration of the stochastic gradient descent. However, such a naive solution will not lead to order optimal convergence rates. 

% This method is inspired from a concept called \emph{re-parametrization of product form distribution using Bethe approximation} \cite{book_martin}. 

%To address this issue, we propose a method called local Gibbs optimization method which will converge to the Bethe approximated fugacities, and at the same time has an order optimal convergence guarantee. The description of our method is as follows. 

We start with the Gibbsian optimization problem corresponding to the optimal fugacities, and approximate this global problem by decoupling it into local optimization problems at each link. The local problems are identical in structure to the global problem, and are referred to as the local Gibbisan problems. The dimension of the local problem at a link is equal to the size of its immediate neighbourhood and hence typically small, and independent of the network size. Therefore these local Gibbsian problems can be efficiently solved in a scalable fashion. The local solutions are then suitably combined to obtain an approximate solution to the global problem.

We prove that the solution of our local Gibbs optimization method corresponds exactly to the celebrated Bethe approximation \cite{yedidia} to the global Gibbsian optimization problem. The accuracy of the Bethe approximation has been empirically evidenced in various fields \cite{bethe_emprical}. Therefore, it is reasonable to expect a fair degree of accuracy in the context of CSMA as well. In fact, numerical results indicate that in order to obtain the level of accuracy in the fugacities obtained by using our proposed method, the stochastic gradient descent method \cite{libin} takes an inordinately long time, often running into tens of millions of time units even for fairly small networks. Therefore, in practical terms, our algorithm will operate with substantially smaller convergence time, compared to the original implementation of adaptive CSMA.
\begin{comment}
%Finally, we address the issue of obtaining a provably throughput optimal CSMA algorithm using our approximation. Although the fugacities obtained using the Bethe approximation correspond closely to the desired service rates in most  practical scenarios, the fugacities are still approximate. In particular, a CSMA algorithm which uses these approximate fugacities is not technically throughput optimal. In order to obtain a provably throughput optimal CSMA algorithm, we simply use the Bethe approximated fugacities as a good initial iterate for the usual stochastic gradient descent.
\end{comment} 

It is worth noting that our algorithm is robust to gradual changes in the desired service rates, as well as to changes in the network topology, since the local solutions can be efficiently re-computed for the new set of requirements. On the other hand, the stochastic gradient descent is likely to take a very long time to converge to its new operating point. 

The impractically slow mixing time of the CSMA Markov chain is also known to result in poor delay performance \cite{hardness, fast_mixing}. Recent works like~\cite{parallel_chains, parallel_chains2} have shown improved  delay performance by employing several parallel instances of this Markov chain. However, the result in \cite{parallel_chains} assumes that the required optimal fugacities can be pre-computed and given to their algorithm. Our local algorithms which efficiently estimate these fugacities can be used in conjunction with the techniques in \cite{parallel_chains, parallel_chains2} to obtain a practical CSMA algorithm with good throughput and delay properties.


%Hence, we remark that the existing CSMA algorithms \cite{parallel_chains} which are known to effectively support the service rates once the fugacities are computed, can be used in conjunction with our proposed method to design a practical CSMA algorithm. 
%
%In summary, the key contributions in this paper are as follows:
% 
% We propose an efficient and scalable method to approximate the fugacities corresponding to the desired service rates, under a realistic SINR model for the interference.
%
% We prove that our local Gibbsian method is exactly equivalent to performing the Bethe approximation for the global Gibbsian optimization problem.
%
%  As special cases of our model, we consider the conflict graph model \cite{bethe_jshin} and the conservative SINR model \cite{sinr_mimo}, and derive closed form expressions for the solutions to the corresponding local problems.
%
%%\item We derive closed form solutions to the local problems for two special cases of our model, which have been studied earlier -- namely a conflict graph model \cite{bethe_jshin}, and a conservative SINR model \cite{sinr_mimo}.
%
% Simulations suggest that the proposed algorithm estimates the fugacities in very few steps under most    practical scenarios, which leads to a drastic improvement in the convergence time.
%
%We  begin by introducing the system model used in the paper. %



The remainder of this paper is organized as follows. In Section \ref{sec_model}, we describe the SINR based interference model, and review the adaptive CSMA algorithm. In Section \ref{local_gibbs}, we introduce the local Gibbsian problems and propose our algorithm for computing the fugacities for a given service rate requirements. Section \ref{preliminaries_bethe} provides a brief review of the Bethe approximation, as relevant to adaptive CSMA. In Section \ref{gibbs_bethe}, we derive our main result which establishes the equivalence between the local Gibbs optimization, and the Bethe approximation. In Section \ref{special_cases}, we consider the conflict graph model as a special case of the SINR model and derive closed-form expressions for the local Gibbsian problems. In Section \ref{util_max}, we propose a local algorithm to solve the utility maximization problem and quantify its performance. In Section \ref{simulations}, we present numerical results to confirm the fast convergence, and Section \ref{conc} concludes the paper.


==> ArXiv Version TON/local_gibbs.tex <==
%In this section, we define the local Gibbsian optimization problems, whose solutions can be suitably combined to approximate the solution to the global Gibbsian problem.
We now introduce some definitions required for the description of the local Gibbsian problems.

\emph{Local schedule:} Let $\x^{(j)} \in \{0,1\}^{\N_j}$, be the set of variables corresponding to the transmission status of the link $j$ and its neighbors, \ie,
%\begin{align*}
$\x^{(j)}:=\left\lbrace x_k \; | \; k \in \N_j  \right\rbrace.$
%\end{align*}
We refer to $\x^{(j)}$ as the \emph{local schedule} at $j$. Further, from \eqref{eq_int1}, it can be observed that the SINR of a link depends only on the local schedule. Hence the SINR at a link $j$ can be viewed as a function of $\x^{(j)}$, \ie, $\gamma_j(\x) = \gamma_j(\x^{(j)})$. Also, recall that a schedule $\x$ is said to be feasible, if all the active links in the schedule meet their required SINR threshold. Thus, $\i(\x \in \mathcal{I})$ can be factorized over the local schedule variables $\{\x^{(j)}\}_{j=1}^N$ as $\i(\x \in \mathcal{I})= \prod\limits_{j \;: \;x_j=1} \i (\gamma_j(\x^{(j)}) \geq T).$ Then, \eqref{eq_dist} can be written as
\begin{align}
p(\x)&= \frac{1}{Z} \prod\limits_{j \;: \;x_j=1} \lambda_j \i (\gamma_j(\x^{(j)}) \geq T), & \forall \x \in \{0,1\}^N. \label{eq_succint}
\end{align}

\emph{Local feasiblity:} A local schedule $y = [y_k]_{k \in \N_j} \in \left\lbrace 0, 1 \right\rbrace^{\N_j}$ at link $j$ is said to be \emph{feasible}, if either the link $j$ is inactive (\ie, $y_j=0$), or it is active and meets the required threshold SINR \ie, $(y_j=1$ and $\i (\gamma_j(y) \geq T))$. The set of all the feasible local schedules at $j$ is denoted by $\I_j$. It can be observed from \eqref{eq_succint} that $p(\x)$ assigns zero probability to a schedule $\x$ if any of its local schedule is infeasible.
% Also, from \eqref{eq_succint}, it can be observed that the distribution $p(\x)$ assigns zero probability for a schedule $\x$, if it is locally infeasible at any link $j \in \N$.

\emph{Local service rate vector:} Let $\{s_i\}_{i=1}^N$ be the set of service rates of all the links in the network. Then the local service rate vector at link $j$ denoted by $s^{(j)}$ be defined as the set of all the service rates corresponding to link $j$ and its neighbors, \ie, $s^{(j)}:=\left\lbrace s_k \; | \; k \in \N_j  \right\rbrace.$

\emph{Local capacity region:} The local capacity region at link $j$ is defined as the convex hull of the local feasible schedules at link $j$ given by
\begin{align}
\Lambda_j= \{ \sum_{ z \in \mathcal{I}_j} \alpha_{z} z \; | \; \sum_{z\in \mathcal{I}_j} \alpha_{z}=1, \; \alpha_{z} \geq 0, \; z \in \mathcal{I}_j \}. \label{eq_loc_cap}
\end{align}
Now, we define the local Gibbsian problem at link $j$ as follows:
\begin{align}
\lf_{j} = \arg\max\limits_{r \in \R^{\N_j}} F(r), \label{opt_local_alternate0}
\end{align} 
where $\lf_j:=[\lf_{jk}]_{k \in \N_j}$, and the function $F: \R^{\N_j} \rightarrow \R$ is
\begin{align*}
F(r):=\sum\limits_{k \in \N_j} s_k r_{k} - \ln \Big(\sum\limits_{y \in \I_j} \exp\Big(\sum\limits_{k \in \N_j} y_k r_{k} \Big)\Big).
\end{align*} 
Observe that, the local problems are structurally similar to the global problem, except that $\I$ in the global problem is replaced by $\I_j$, and $\N$ is replaced by $\N_j$. In particular, the dimension of the local problem at link $i$ is just $|\N_i|$. The solutions to these local problems are referred to as the \emph{local fugacities}. In particular, at each link $j \in \N$, there is a local fugacity vector  $\lf_j:=[\lf_{jk}]_{k \in \N_j}$.

\emph{Local algorithm:}
Here, we propose a simple and distributed algorithm (Algorithm 1) to solve the local Gibbsian problems and subsequently compute the approximate global fugacities by combining the local solutions using \eqref{eq_lf_gf0}. These approximate global fugacities can be directly used in the CSMA algorithm instead of adapting the fugacties using a stochastic gradient descent on the global problem which usually doesn't converge in practical time scales. Each link in the network executes the following algorithm in parallel.
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Algorithm 1:} Local Gibbsian method at link $j$\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\; \; \emph{Input:} ($s_{k}$,  $k \in \nj$); \hspace{0.25cm}
\emph{Output:} $\lt_j$.
\begin{enumerate}
\item Obtain the service rates ($s_{k}$,  $k \in \nj$) from the neighbours.
\item Compute the local fugacities ($\lf_{jk}$,  $k \in \nj$) by solving the local problem \eqref{opt_local_alternate0}  using the Newton's method.
\item From each neighbour $k \in \N_j$, obtain the local fugacity $\lf_{kj}$.
\item Compute the approximate global fugacity $\lt_j$ as
\begin{align}
\lt_j&= \left(\frac{1-s_j}{s_j}\right)^{|\N_j|-1}\prod\limits_{k \in \N_j} e^{\lf_{kj}}. \label{eq_lf_gf0}
\end{align}
\end{enumerate}
\noindent\rule[0.5ex]{\linewidth}{0.5pt}

\emph{Information exchange:} The algorithm requires only two steps of information exchange with the neighbours. Once in the first step, to obtain the service requirements of the neighbours, and again in the third step to obtain the local fugacities computed at the neighbours. Except for these two information exchanges, the algorithm is fully distributed and can be executed independently at each link.

\emph{Computational complexity:}
The implementation of the Newton's method \cite[Section 9.5]{boyd} in the second step of our algorithm is feasible. This is because the gradient and the Hessian of the local objective function $F(r)$ can be analytically computed since the dimension of the problem is small. The exact expressions for the gradient and Hessian at link $j$ can be computed using certain marginals of the distribution  $\b_j(\x^{(j)}) =  {Z_j^{-1}} \exp (\sum_{k \in \N_j} x_k r_k ),  \forall \x^{(j)} \in \I_j$, where $Z_j$ is a normalization constant. 

For $k \in \N_j$, let $m_k(r)$ represent the probability $\P(x_k=1)$ under the distribution $\b_j$. Similarly, for $i,k \in \N_j$, let $m_{ik}(r)$ denote the probability $\P(x_i=1, x_k=1)$ under the same distribution $\b_j$. 
Then, the gradient and Hessian of the function $F(r)$ are given by
\begin{align*}
[\nabla(F(r))]_k&= s_k-m_k(r), \; \;  k \in \N_j, \\
[\nabla^2(F(r))]_{ik}&= \begin{cases}
m_{ik}(r)-m_i(r)m_k(r) , \; \;  i,k \in \N_j, i \neq k\\
m_k(r)-m_k(r)^2, \; \; i=k.
\end{cases}
\end{align*}
The computation of the gradient and the Hessian requires the information about the local feasible schedules at a link. Specifically, this information is required to compute the normalization constant $Z_j$.  These computations are feasible because the $O(2^{|\N_j|})$ complexity involved in this computation scales only with the size of the local neighborhood, and is independent of the total size of the network which could be substantially large. In particular, in spatial networks where the neighborhood size does not scale with the network size, our algorithm is order optimal.
%\begin{comment}
%Let $g(t)$, $H(t)$ denote the gradient and Hessian at $r(t)$.
%
%%\emph{Algorithm2} essentially solves the following unconstrained optimization problem in $\R^{\nii}$.
%%\begin{align}
%% \arg\max\limits_r K(r), \label{local_opt}
%%\end{align}
%% where,
%%\begin{align*}
%%K(r):&=\sum\limits_{j \in \nii} s_j r_{j} - \log \left(\sum\limits_{\rho \in \mathcal{F}_i} \exp\left(\sum\limits_{j \in \nii} \rho_j r_{j} \right)\right)
%%\end{align*}
%\noindent\rule[0.5ex]{\linewidth}{0.5pt}
%\emph{Algorithm2}:\\ \textbf{Newtons method at link $j$ to compute local fugacities}\\
%\noindent\rule[0.5ex]{\linewidth}{0.5pt}
%\; \; \textbf{Input:} ($s_{j}$,  $j \in \ni$); \hspace{0.25cm}
%\textbf{Output:} ($\lf_{ij}$,  $j \in \ni$).
%\begin{enumerate}
%\item Set $t=1$ and initialize $r(1)$ to zero.
%
%\item Compute the gradient $g(t)$ and the Hessian $H(t)$.
%
%\item Update $r(t+1)= r(t) + H(t)^{-1}g(t)$. 
%\item Repeat steps 2,3 till gradient is close to zero.
%\end{enumerate}
%\noindent\rule[0.5ex]{\linewidth}{0.5pt}
%
%
%\emph{Remark:} In the second step of \emph{Algorithm2}, the link should compute the $H(t)$ and $g(t)$ analytically. This computation is feasible because the dimension of the problem is just the number of neighbours, which is reasonably small in most practice cases.
%\end{comment}

In Section \ref{gibbs_bethe}, we prove that the approximate global fugacites $\{\lt_j\}_{j=1}^N$ obtained using the local Gibbsian method \eqref{eq_lf_gf0} correspond exactly to performing the well known Bethe approximation to the global Gibbsian problem. In the next section, we review the Bethe approximation technique.

==> ArXiv Version TON/numerical_results_new.tex <==
\begin{figure*} %Random topology
\begin{subfigure}{.33 \textwidth}
\centering
\includegraphics[scale=0.28]{rk.pdf} 
\caption{15-link random topology} %fifteen link network used for simulations. Each node represents a link in the network. An edge is present if two links are in the interference range.}
\label{fig_rg15}
\end{subfigure}
\begin{subfigure}{.33 \textwidth}
\centering
\includegraphics[scale=0.34]{rg_20nodes.pdf} 
\caption{20-link random topology} %fifteen link network used for simulations. Each node represents a link in the network. An edge is present if two links are in the interference range.}
\label{fig_rg20}
\end{subfigure}
\begin{subfigure}{.33 \textwidth}
\centering
\includegraphics[scale=0.34]{grid_topology.pdf}
\caption{4 $\times$ 4 grid topology}
\label{fig_grid_graph}
\end{subfigure}
\caption{Illustration of some interference graphs used: Each vertex represents a link in the network. An edge is present if two links are in the interference range.}
\label{fig_all}
\end{figure*}




\begin{figure*}
\begin{subfigure}{.5 \textwidth}
\centering
%\includegraphics[scale=0.45]{fig_error_new_v3.eps} 
\includegraphics[scale=0.38]{15and20_link_comparision.pdf} 
\caption{Error as a function of target service rate for the random topologies}
\label{fig_be_load_20}
\end{subfigure}
\begin{subfigure}{.5 \textwidth}
\centering
%\includegraphics[scale=0.43]{two_versions_sdg_load8_20p.eps}
\includegraphics[scale=0.4]{time_comparision_all3.pdf}
\caption{Error as a function of time for 20-link random graph}
\label{fig_time}
\end{subfigure}
\caption{Comparision of errors due to SGD and our Bethe approximation based algorithms for random topologies in Figure \ref{fig_all}}
\end{figure*}

\begin{figure*}
\begin{minipage}{.5 \textwidth}
\centering
%\includegraphics[scale=0.25]{time0.eps} two_versions_sdg_load8_20p.pdf
\includegraphics[scale=0.38]{completegraph_2sizes.pdf} 
\caption{Bethe error for complete graph topology}
\label{fig_completegraph_error}
\end{minipage}
\begin{minipage}{.5 \textwidth}
\centering
\includegraphics[scale=0.4]{grid_both_sizes_till9.pdf}
\caption{Bethe error for grid topology}
\label{fig_gridgraph_error}
\end{minipage}
\end{figure*}


%\begin{comment}
\begin{figure}
\centering
\includegraphics[scale=0.46]{fig_umax_two.pdf} 
\caption{Convergence of local utility maximization algorithm}
\label{fig_umax}
\end{figure}
%\end{comment}
\begin{comment}
\begin{figure}
\centering
\includegraphics[scale=0.4]{ton_plot_queues.pdf} 
\caption{Comparison of queue length performance using $10 \times 10$ grid topology.  Here, `Bethe approx' corresponds to using the Bethe approximation with traditional CSMA (only single Markov chain) \cite{libin}; `Bethe + parallel' corresponds to using the Bethe approximation proposed in this paper with $10$ parallel CSMA Markov chains \cite{parallel_chains2};}
\label{fig_queues}
\end{figure}
\end{comment}
In this section, we present simulations to evaluate the performance of our algorithms. We consider three topologies namely random graphs, complete graph, and grid graph.
\subsection{Bethe error}
\emph{Simulation setting for random graphs:} We generate a spatial random network by uniformly placing the transmitter nodes on a two dimensional square plane of length $8$.  Each transmitter is associated with a receiver at a distance of $0.5$ in a random direction. The path loss exponent $\alpha$ is set to $3$, the close-in radius $R_I$ is set to $2.4$, and the threshold SINR is set to $15$ dB. The transmit power of the links is set to $1$. We consider equal service rate requirements for all the links. For a given target service rate vector $s^t=[s_i^t]_{i=1}^N$,  we define the Bethe approximation error as 
\begin{align*}
e(s^t)= \frac{\sum_{i=1}^N  |s^t_i - s^a_i|}{N},
\end{align*}
where $s^a=[s_i^a]_{i=1}^N$ are the service rates that can be supported by the approximated fugacities $\{\lt\}_{i=1}^N$. 

\emph{Bethe error as function of target service rate:}
We generated two random networks of sizes $15$ and $20$ links (shown in Figure \ref{fig_rg15}, \ref{fig_rg20}). We compared the error of our approximation algorithm with the residual error of the SGD algorithm \cite{libin} after running the SGD for $10^{8}$ time-slots of the CSMA algorithm. In Figure \ref{fig_be_load_20}, we plot the approximation error as a function of the target service rate. Further, for the considered SINR constraints, we numerically observed that for both the random topologies in Figure \ref{fig_all}, CSMA can support till a  service rate of $0.33$ for all the links. Hence, we varied the target service rate from $0$ to $0.33$. It can be observed from Figure \ref{fig_be_load_20}, that for practical time-scales, our algorithm results in better accuracy than the SGD for all the target service rates.

 


\emph{Error as a function of time:} In Figure \ref{fig_time}, for a fixed target service rate of  $0.25$, we plot the approximation error as a function of time, by using the time-averaged service rates observed from CSMA algorithm. Here, our local Gibbs algorithm computes the Bethe approximated fugacities, and uses these static fugacities (\ie, they are not adapted during the algorithm) in the CSMA algorithm. The SGD algorithm starts with some initial fugacities, and adapts the fugacities by observing the corresponding service rates. We simulated two versions of the SGD algorithm (SGD-1, SGD-2) proposed in \cite{libin,libin_arxiv}, whose details are as follows: The update rule of SGD algorithm has two functions to be chosen, namely update interval $T(j)$, and step size $\alpha(j)$, for the $j^{th}$ iteration of the gradient descent. The update rule for SGD-1 \cite[Section II-D]{libin} is given by $\alpha(j)=\frac{1}{(j+2)\log(j+2)}$, $T(j)=j+2$. The update rule for SGD-2 \cite[Scheduling Algorithm 1]{libin_arxiv} is given by $\alpha(j)=\frac{1}{j}$, $T(j)=\exp(\sqrt{j})$. 

Although the SGD algorithm will eventually converge to the exact fugacities, from Figure \ref{fig_time}, it can be observed that for practical time-scales of the order of $10^8$ time slots, the residual error is rather large compared to our approximation algorithm. This is because, the CSMA Markov chain has to mix only one time for the Bethe approximation based approach, as the fugacities are static. However, in the SGD based approach, for every update in the fugacities, the Markov chain tries to mix to a new steady state distribution.



\emph{Complete graph and Grid graph:}
Here, we consider two complete graph topologies with sizes $15$ and $20$, and two grid topologies of sizes $16$ and $25$. A $4 \times 4$ grid topology is illustrated in Figure \ref{fig_grid_graph}.  The range of the target service rates is chosen by numerically observing the maximum supportable service rates for the respective topologies. We plot the Bethe error for these two topologies as a function of the target service rates in Figure \ref{fig_completegraph_error}, \ref{fig_gridgraph_error}. As seen from the plots, the error is considerably small for both the topologies.

%\begin{comment}
\subsection{Convergence of Utility maximization algorithm}
Here, we consider the case of computing the fugacities for the proportional fairness utility setting, \ie, $U_i(s_i)= \log s_i$ for all the links. We update the fugacities using Algorithm 2 proposed in Section \ref{util_max}. In Figure \ref{fig_umax}, we plot the norm of the subgradient corresponding to the  maximization problem \eqref{eq_util_bethe}, which indicates the convergence of the algorithm. The convergence is plotted for the two random topologies of size $15$ and $20$. It can be observed that the proposed algorithm converges within 200 iterations.  
%\end{comment} 



 %As seen from the plots, the Bethe error is considerably small for all the target service rates except for the very high load regime.

%\subsection{Delay Performance} The impractically slow mixing time of the CSMA Markov chain is also known to result in poor delay performance \cite{hardness, fast_mixing}. Recent works like~\cite{parallel_chains, parallel_chains2} have improved the delay performance by employing several parallel instances of the CSMA Markov chain. These results \cite{parallel_chains} are proved under the assumption that the optimal fugacities are pre-computed, and are readily available to the algorithm. Our local algorithms which efficiently estimate these fugacities, can be used in conjunction with the techniques in \cite{parallel_chains, parallel_chains2} to obtain a practical CSMA algorithm with good throughput and delay. %We demonstrate this idea by using a $10 \times 10$ grid topology in our supplementary material. 
%%\begin{comment}
%
%We demonstrate this idea by using a $10 \times 10$ grid topology. Here, we assume that each link has a Bernoulli arrival process, and plot the time average queue length in Figure \ref{fig_queues} after running the CSMA algorithm for $10^7$ slots. We compared the following approaches in the literature. We have simulated the SGD algorithm \cite{libin}, queue-length based adaptive CSMA (Q-CSMA) \cite{qcsma}, and our Bethe approximation based CSMA algorithm.  The details of Q-CSMA algorithm used: Different weights for Q-CSMA have been proposed in literature. We have considered the weight $\log(0.1q)$ proposed in \cite{qcsma}. The results are qualitatively similar for other choices of weights. As seen from Figure \ref{fig_queues}, for arrival rates above $0.2$,  the queue lengths under the above three algorithms are rather large.
%
%However, if we use the Bethe approximation algorithm proposed in this paper in conjunction with parallel chain based CSMA \cite{parallel_chains}, the queue length performance is significantly improved. For example, the queue length is quite low even at a reasonably large arrival rate of $0.35$.
%%\end{comment}

==> ArXiv Version TON/preliminaries.tex <==
%\begin{comment}
%\subsubsection*{Factor graph}
%Consider a product-able function $f(x)$ given by,
%\begin{align*}
%f(x_1,x_2,x_3,x_4,x_5)= f_1(x_1, x_2 , x_5) f_2(x_2, x_4) f_3(x_3, x_5).
%\end{align*}
% A factor graph \cite{yedidia} is a bipartite graph, that captures the factorization of a product-able function like $f(x)$. The factor graph has a set of nodes called \emph{variable nodes} corresponding to the variables of the function $f$. The graph has another set of nodes called \emph{factor nodes}, corresponding to the functions in the product. The variable nodes are represented using circles while the factor nodes are represented using squares.  An edge is drawn between a variable node a factor node if that variable is an argument of the factor node. For example, the factor graph of the considered function $f(x)$ is given by Figure \ref{fig_fg}.
%
%
%\subsection{Gibbs free energy}
%Let us consider the following concept of Boltzmann law from statistical physics. In a system with $N$ particles, the state of each particle is denoted by a random variable $X_i$, and the overall state of the system is specified a vector $X$. The free energy of a particular state of the system $x \in S$, where $S$ is state space of the system, is given by a energy function $E(x)$. The probability distribution on the state of the system in thermal equilibrium is given by the Boltzmann law as follows.
%\begin{align}
%p(x)&= \frac{1}{Z(T)}e^-{\frac{E(x)}{T}}, & \forall x \in S,
%\end{align}
%where, T is the temperature of the system, and $Z(T)$ is the normalization constant, which is also referred as partition function is given by,
%\begin{align*}
%Z(T)= \sum\limits_{x \in S} e^{-\frac{E(x)}{T}}.
%\end{align*}
%If we consider a non-physical system, we can still define an analogous energy function as follows. Consider a distribution on the random vector $X$, which is product-able into $M$ factors as given by,
%
%Consider a set of $N$ discrete-valued random variables namely $\{ X_1, X_2, \dots, X_N \}$. The possible realizations of a random variable $X_i$ is denoted by $x_i$. Let $S$ denote the state space of a random variable $X_i$, which is same for all the random variables. The joint PMF (probability mass function) of the random variables is succinctly denoted as,
%\begin{align*}
%p(\x)= p(X_1=x_1, X_2=x_2, \dots, X_N = x_N),
%\end{align*}
%where $\x=\{x_1,x_2, \dots, x_N \}$.
%
%Suppose $p(\x)$ factors into a product of $M$ functions given by,
%\begin{align}
%p(\x)&= \frac{1}{Z} \prod\limits_{j=1}^M f_j(\x^{(j)}), \hspace{0.7cm} \x \in S^N.  \label{eq_factors}
%\end{align}
%The function $f_j(\cdot)$ has arguments $\x^{(j)}$ that are some subset of $\{x_1,x_2, \dots, x_N \}$. The functions are assumed to be non-negative and finite, so that the PMF is well defined. Here $Z$ is the normalization constant. Let us now consider an example.
%\begin{figure}
%{
%\begin{center}
%\begin{tikzpicture}[scale=0.3]
%\draw (0,0) -- (-2,0.7);
%\draw (-2,-0.7) -- (0,0);
%\draw (0,0) -- (0.7,0);
%\draw (0.7,0) -- (0.7,0.7);
%\draw (0.7,0.7) -- (0,0.7);
%\draw (0,0.7) -- (0,0);
%\node at (0.35,-0.7) {{$f_1$}};
%
%\draw (2,0) -- (2.7,0);
%\draw (2.7,0) -- (2.7,0.7);
%\draw (2.7,0.7) -- (2,0.7);
%\draw (2,0.7) -- (2,0);
%\node at (2.35,-0.7) {{$f_2$}};
%
%\draw (4,0) -- (4.7,0);
%\draw (4.7,0) -- (4.7,0.7);
%\draw (4.7,0.7) -- (4,0.7);
%\draw (4,0.7) -- (4,0);
%\node at (4.35,-0.7) {{$f_3$}};
%
%
%\draw (-1.5,3)circle(0.4cm);
%\node at (-1.5,4) {{$x_1$}};
%\draw (0.5,3)circle(0.4cm);
%\node at (0.5,4) {{$x_2$}};
%\draw (2.5,3)circle(0.4cm);
%\node at (2.5,4) {{$x_3$}};
%\draw (4.5,3)circle(0.4cm);
%\node at (4.5,4) {{$x_4$}};
%\draw (6.5,3)circle(0.4cm);
%\node at (6.5,4) {{$x_5$}};
%\node at (3,0.85+0.2) {$2$};
%
%
%
%
%
%\draw (0.35,0.7) -- (-1.5,3-0.4); %A- x1
%\draw (0.35,0.7) -- (0.5,3-0.4); %A- x2
%\draw (0.35,0.7) -- (6.5,3-0.4); %A- x5
%
%\draw (2.35,0.7) -- (0.5,3-0.4); %B- x2
%\draw (2.35,0.7) -- (4.5,3-0.4); %B- x4
%
%%\draw (4.35,0.7) -- (-1.5,3-0.4); %C- x1
%\draw (4.35,0.7) -- (2.5,3-0.4); %C- x3
%\draw (4.35,0.7) -- (6.5,3-0.4); %C- x5
%\end{tikzpicture}
%\end{center}
%}
%\vspace{-0.6cm}
%\caption{Factor graph}
%\label{fig_fg}
%\end{figure}
%
%\textbf{Example} (A simple factor graph): Consider a simple distribution given by,
%\begin{align*}
%p(x_1,x_2,x_3,x_4,x_5)&= \frac{1}{Z} f_1(x_1, x_2 , x_5) f_2(x_2, x_4) f_3(x_3, x_5).
%\end{align*}
%Using the notation in \eqref{eq_factors}, the distribution can be succinctly represented as,
%\begin{align}
%p(\x)&= \frac{1}{Z} f_1(\x^{(1)}) f_2(\x^{(2)}) f_3(\x^{(3)}), \label{eq_example_prod}
%\end{align}
%where, $\x=\{x_1, x_2, x_3, x_4, x_5 \}$, $\x^{(1)}=\{x_1, x_2,  x_5 \}$, $\x^{(2)}=\{ x_2,  x_4 \}$, $\x^{(3)}=\{x_3,  x_5 \}$.
%\subsubsection*{Factor Graph}
%A factor graph \cite{yedidia} is a bipartite graph, that is used to visualize the factorization structure of distribution \eqref{eq_factors}. The factor graph has a set of nodes called \emph{variable nodes} corresponding to the variables $\{x_1,x_2, \dots, x_N \}$. It also has another set of nodes called \emph{factor nodes}, corresponding to the functions in \eqref{eq_factors}. The variable nodes are represented using circles while the factor nodes are represented using squares.  An edge is drawn between a variable node a factor node if that variable is an argument of the factor node. For example, the factor graph of the distribution considered in \eqref{eq_example_prod} is given by Figure \ref{fig_fg}.
%\subsubsection*{Marginal probability functions}
%For the product form distribution considered in \eqref{eq_factors}, we are interested in the marginal probability functions called variable marginals and factor marginals. Here, $p_i$ represents the marginal corresponding to the variable node $i$, while $\p_i$ represent the marginal corresponding to the factor node $i$.
%\begin{itemize}
%\item[(i)]  \emph{Variable node marginals: $p_i(x_i)$}\\
%The marginal probability function $p_i({x_i})$ corresponding to each variable node $i$, is obtained by summing $p(\x)$ over the variables corresponding to all other variable nodes.
%\begin{align*}
%p_i({x_i}) &= \sum\limits_{\x \setminus x_i} p(\x), &x_i \in S, \;  i=1 \text{ to } N.
%\end{align*}
%Let $\pv:=\{p_i\}_{i=1}^N$ denote the collection of all the variable node marginals corresponding to the distribution $p(\x)$.
%\item[(ii)] \emph{Factor node marginals: $\p_j(\x^{(j)})$}\\ 
%Corresponding to each factor node, $j=1 \text{ to } M$, the marginal probability function $\p_j({\x^{(j)}})$,  is obtained by summing $p(\x)$ over all the variables in $\x \setminus \x^{(j)}$. Let $N_j$ denote the number of arguments in $f_j$, \ie, $N_j= |\x^{(j)}|$.
%\begin{align*}
%\p_{j}({\x^{(j)}}) = \sum\limits_{\x \setminus \x^{(j)}} p(\x), \; \; \; \; \x^{(j)} \in S^{N_j}.
%\end{align*}
%Let $\pn:=\{\p_j\}_{j=1}^M$ denote the collection of all the factor node marginals corresponding to the distribution $p(\x)$.
%\end{itemize}
%As discussed earlier, the computation of the marginal probability distributions requires the computation of the partition function $Z$, which is a NP-hard problem \cite{bremaud}. Next, we discuss a technique called Bethe approximation which is used to estimate the marginal probability distributions. 
%\subsection{Bethe approximation}
%One approach to compute the partition function corresponding to the distribution $p(\x)$,  is to minimize a function called Gibbs free energy (GFE) over all the valid probability distributions on the state space $S^N$. However, as $N$ becomes large, even this procedure is intractable, as the optimization variables take exponentially large memory to store.  Moreover, this method only computes the partition function, but doesn't explicitly compute the marginals. We hence take recourse to the Bethe approximation, which is an approximate, but a more practical technique to estimate the marginals explicitly.
%We begin with the definition of energy function. (Note that, we define these concepts of free energy with focus on the application for CSMA networks. For a general and detailed discussion, the readers are referred to \cite{yedidia}.)
%\begin{definition}
%For a distribution $p(\x)$ in the form of \eqref{eq_factors}, the energy function $E(\x) : S^N \rightarrow \R$ is defined as,
%\begin{align*}
%E(\x)= - \sum\limits_{j=1}^{M} \ln f_j(\x^{(j)}).
%\end{align*}
%\end{definition}
%Observe that the energy function $E(\x)$ completely specifies the distribution $p(\x)$ in \eqref{eq_factors}, as follows:
%\begin{align*}
%p(\x)&= \frac{1}{Z} e^{-E(\x)}, \hspace{0.5cm} \x \in S^N,
%\end{align*}
%where, the partition function is given by $Z= \sum\limits_{\x \in S^N} e^{-E(\x)}$.
%
%Next, we shall define the terms Bethe free energy (BFE) and Bethe optimization (BO).
%\begin{definition}
%Consider an energy function $E(\x)$ which corresponds to a true distribution $p(\x)$. Let $b(\x)$ be a trial distribution. Then the Gibbs free energy $F_G(b)$, is defined as,
%\begin{align}
%F_G(b)= U_G(b) - H_G(b),
%\end{align}
%where, $U(b)$ is the average energy of the system under the distribution $b(\x)$ given by,
%\begin{align}
%U_G(b)=\sum\limits_{\x \in S^N} b(\x) E(\x),
%\end{align}
%and $H_G(b)$ is the entropy of the system under the distribution $b(\x)$ given by,
%\begin{align}
%H_G(b)= - \sum\limits_{\x \in S^N} b(\x) \ln b(\x).
%\end{align}
%\end{definition}
%
%(Note that we compute the entropy using the natural logarithm instead of the usual base-2 logarithm in order to be consistent with the physics literature.)
%
%
%The partition function corresponding to $p(x)$, can be computed by solving the following optimization namely Gibbs free energy minimization :
%\begin{align}
%- \ln Z = \min\limits_b F_G(b). \label{eq_gibbs_min}
%\end{align}
%Moreover, if the minimum is achieved at $b^*$, then 
%\begin{align*}
%p(\x)=b^*(\x), \; \;  \; \forall \x \in S^N.
%\end{align*}
%Here, the optimization is done over all the possible distributions on $S^N$. 
%Bethe approximation does two approximations for the optimization problem considered in \eqref{eq_gibbs_min}. First, the GFE $F_G(b)$ is approximated using the Bethe free energy (BFE) $F_B(b)$, defined in \eqref{eq_bfe_eg}. Second, the optimization of the BFE is performed over a restricted set, which will be described in \eqref{eq_bethe_min}.
%
%\end{comment}

 We now introduce some terminology required to describe the Bethe approximation technique \cite{yedidia}. 
\subsection{Product form distribution}
Let $S$ be a finite set, and let $X_i, i=1, 2, \dots, N$, be random variables each taking values in $S$. The joint PMF (probability mass function) of the random variables is succinctly denoted as $p(\x)$, where $\x=\{x_1,x_2, \dots, x_N \}$. Suppose that $p(\x)$ factors into a product of $M$ functions and is given by,
\begin{align}
p(\x)&= \frac{1}{Z} \prod\limits_{j=1}^M f_j(\x^{(j)}), \hspace{0.7cm} \x \in S^N.  \label{eq_factors}
\end{align}
The function $f_j(\cdot)$ has arguments $\x^{(j)}$ that are some non-empty subset of $\x=\{x_1,x_2, \dots, x_N \}$. Here $Z$ is a normalization constant. Further, the product form distributions are generally represented using a graph called factor graph \cite{yedidia} that has two sets of nodes namely variable nodes and factor nodes corresponding to the variables and the functions in \eqref{eq_factors} respectively. An edge is drawn between a variable node and a factor node if the variable is an argument of that factor function.

For the product form distribution considered in \eqref{eq_factors}, we are interested in certain marginal probabilities called the variable marginals and the factor marginals.

\noindent \emph{Variable node marginals: }
The marginal probability distribution $p_i({x_i})$ corresponding to a variable node $i$, is obtained by summing $p(\x)$ over the variables corresponding to all other variable nodes, \ie, $p_i({x_i})= \sum_{\x \setminus x_i} p(\x)$, $x_i \in S$, $ i=1,\dots, N.$

\noindent \emph{Factor node marginals:} Corresponding to each factor node, $j=1, \dots, M$, the marginal probability function $\p_j({\x^{(j)}})$,  is obtained by summing $p(\x)$ over all the variables in $\x \setminus \x^{(j)}$. Let $N_j$ denote the number of arguments in $f_j$, \ie, $N_j= |\x^{(j)}|$. Then, 
$
\p_{j}({\x^{(j)}}) = \sum_{\x \setminus \x^{(j)}} p(\x)$, $\x^{(j)} \in S^{N_j}.$

Let $\pv:=\{p_i\}_{i=1}^N$, $\pn:=\{\p_j\}_{j=1}^M$ denote the collection of all the variable node marginals and  the factor node marginals corresponding to the distribution $p(\x)$ respectively. 


The computation of these marginal probability distributions requires the computation of the normalization constant $Z$, which is an NP-hard problem \cite{yedidia}. Next, we discuss the notions of Gibbs free energy (GFE) and the Bethe free energy (BFE) which provide a variational characterization of the normalization constant and the marginal distributions.

 
\subsection{Gibbs free energy}
Consider a probability distribution $p(\x)$ of the form \eqref{eq_factors} for which we are interested in finding the normalization constant $Z$, and the marginals. Let $b(\x)$ be some distribution on $S^N$. Here, $p(\x)$ is referred to as the \emph{true} distribution, and $b(\x)$ is referred to as the \emph{trial} distribution as it will be used to estimate the true distribution $p(\x)$.
%One approach to compute the partition function corresponding to the distribution $p(\x)$,  is to minimize a function called Gibbs free energy (GFE) over all the valid probability distributions on the state space $S^N$. However, as $N$ becomes large, even this procedure is intractable, as the optimization variables take exponentially large memory to store.  Moreover, this method only computes the partition function, but doesn't explicitly compute the marginals. We hence take recourse to the Bethe approximation, which is an approximate, but a more practical technique to estimate the marginals explicitly.
We now introduce the notion of energy function which is required to define the Gibbs free energy \cite{yedidia}. For a given distribution $p(\x)$ in the form of \eqref{eq_factors}, the energy function $E(\x) : S^N \rightarrow \R$ is defined as $E(\x)= - \sum_{j=1}^{M} \ln f_j(\x^{(j)}).$ Observe that the energy function $E(\x)$ completely specifies the distribution $p(\x)$ in \eqref{eq_factors}, as $p(\x)= \frac{1}{Z} e^{-E(\x)}.$ Using the definition of the energy function, the GFE can be defined as follows. 
%Next, we shall define the terms Bethe free energy (BFE) and Bethe optimization (BO).
\begin{definition}
Consider an energy function $E(\x)$ which corresponds to a true distribution $p(\x)$. Let $b(\x)$ be a trial distribution. Then the Gibbs free energy $F_G(b)$ is defined as $F_G(b)= U_G(b) - H_G(b)$, where the term $U_G(b)=\sum_{\x \in S^N} b(\x) E(\x)$ is called the average energy, and $H_G(b)= - \sum_{\x \in S^N} b(\x) \ln b(\x)$ is the entropy of the distribution $b(\x)$.
\end{definition}
The GFE provides a variational characterization of the normalization constant $Z$ of $p(\x)$ as $- \ln Z = \min_b F_G(b).$ Further, if the minimum of $F_G(b)$ is achieved at $b^*$, then $p(\x)=b^*(\x), \; \forall \x \in S^N.$ 

Here, the optimization is over all the possible distributions on $S^N$. However, as $N$ becomes large, this procedure is intractable, as the optimization variables take exponentially large memory to store.  Moreover, this method only computes the partition function, but doesn't explicitly compute the marginals. We hence take recourse to the Bethe approximation, which is an approximate, but a more practical technique to estimate the marginals explicitly. In particular, the Bethe approximation does two approximations: First, the GFE $F_G(b)$ is approximated using the BFE $F_B(b)$ defined in \eqref{eq_bfe_eg}. Second, the optimization of the BFE is performed over a restricted set of distributions, which will be described in \eqref{eq_bethe_min}. 



%\begin{comment}
%\textbf{Factor graph:}
%A factor graph \cite{yedidia} is a bipartite graph used to visualize the factorization structure of the joint distribution \eqref{eq_factors}. The factor graph has two sets of nodes called the \emph{variable nodes} and the \emph{factor nodes} corresponding to the variables and the functions in \eqref{eq_factors} respectively. The variable nodes are represented using circles while the factor nodes are represented using squares. An edge is drawn between a variable node and a factor node if the variable is an argument of that factor function.
%  Let us now consider an example.\\
%\begin{figure}
%{
%\begin{center}
%\begin{tikzpicture}[scale=0.3]
%%\draw (0,0) -- (-2,0.7);
%%\draw (-2,-0.7) -- (0,0);
%\draw (0,0) -- (0.7,0);
%\draw (0.7,0) -- (0.7,0.7);
%\draw (0.7,0.7) -- (0,0.7);
%\draw (0,0.7) -- (0,0);
%\node at (0.35,-0.7) {{$f_1$}};
%
%\draw (2,0) -- (2.7,0);
%\draw (2.7,0) -- (2.7,0.7);
%\draw (2.7,0.7) -- (2,0.7);
%\draw (2,0.7) -- (2,0);
%\node at (2.35,-0.7) {{$f_2$}};
%
%\draw (4,0) -- (4.7,0);
%\draw (4.7,0) -- (4.7,0.7);
%\draw (4.7,0.7) -- (4,0.7);
%\draw (4,0.7) -- (4,0);
%\node at (4.35,-0.7) {{$f_3$}};
%
%
%\draw (-1.5,3)circle(0.4cm);
%\node at (-1.5,4) {{$x_1$}};
%\draw (0.5,3)circle(0.4cm);
%\node at (0.5,4) {{$x_2$}};
%\draw (2.5,3)circle(0.4cm);
%\node at (2.5,4) {{$x_3$}};
%\draw (4.5,3)circle(0.4cm);
%\node at (4.5,4) {{$x_4$}};
%\draw (6.5,3)circle(0.4cm);
%\node at (6.5,4) {{$x_5$}};
%%\node at (3,0.85+0.2) {$2$};
%
%
%
%
%
%\draw (0.35,0.7) -- (-1.5,3-0.4); %A- x1
%\draw (0.35,0.7) -- (0.5,3-0.4); %A- x2
%\draw (0.35,0.7) -- (6.5,3-0.4); %A- x5
%
%\draw (2.35,0.7) -- (0.5,3-0.4); %B- x2
%\draw (2.35,0.7) -- (4.5,3-0.4); %B- x4
%
%%\draw (4.35,0.7) -- (-1.5,3-0.4); %C- x1
%\draw (4.35,0.7) -- (2.5,3-0.4); %C- x3
%\draw (4.35,0.7) -- (6.5,3-0.4); %C- x5
%\end{tikzpicture}
%\end{center}
%}
%\vspace{-0.6cm}
%\caption{Factor graph}
%\label{fig_fg}
%\end{figure}
%\emph{Example} (A simple factor graph): Consider a simple distribution of the form
%\begin{align*}
%p(x_1,x_2,x_3,x_4,x_5)&= \frac{1}{Z} f_1(x_1, x_2 , x_5) f_2(x_2, x_4) f_3(x_3, x_5).
%\end{align*}
%Using the notation in \eqref{eq_factors}, the distribution can be succinctly represented as
%\begin{align*}
%p(\x)&= \frac{1}{Z} f_1(\x^{(1)}) f_2(\x^{(2)}) f_3(\x^{(3)}), 
%\end{align*}
%where, $\x=\{x_1, x_2, x_3, x_4, x_5 \}$, $\x^{(1)}=\{x_1, x_2,  x_5 \}$, $\x^{(2)}=\{ x_2,  x_4 \}$, $\x^{(3)}=\{x_3,  x_5 \}$. The factor graph corresponding to this example is shown in Figure \ref{fig_fg}.\\
%\end{comment}

\subsection{Bethe approximation}
%One approach to computing the partition function corresponding to the distribution $p(\x)$,  is to minimize a function called Gibbs free energy (GFE) over all the valid probability distributions on the state space $S^N$. However, as $N$ becomes large, even this procedure is intractable, as the optimization variables take exponentially large memory to store. We hence take recourse to the Bethe approximation, which is an approximate, but a more practical technique to estimate the marginals explicitly \cite{yedidia} . Next, we introduce the concepts of Bethe free energy and Bethe optimization with focus on the application for CSMA networks. 
\subsubsection{Bethe free energy (BFE)}
We first define the Bethe entropy of a distribution $b(\x)$, which is a function of the factor and variable marginals of $b(\x)$. The Bethe entropy is given by%$H_B\left( \bn, \bv \right)=\sum_{j=1}^M \H_j(\b_j) - \sum_{i=1}^N (d_i-1) H_i(b_i)$. Here,
\begin{align*}
H_B\left( \bn, \bv \right)
&=\sum\limits_{j=1}^M \H_j(\b_j) - \sum\limits_{i=1}^N (d_i-1) H_i(b_i).
\end{align*}
Here, $d_i$ is the degree of the variable node $i$ in the factor graph, and $\H_j(\b_j)= -\sum_{y \in S^{N_j}} \b_j(y) \ln \b_j(y)$, $
H_i(b_i)= -\sum_{y \in S} b_i(y) \ln b_i(y)$ denote the entropies of the factor marginal $\b_j(\x^{(j)})$, and the variable marginal $b_i(x_i)$ respectively.
\begin{definition}
Consider a true distribution $p(\x)$ of the form \eqref{eq_factors}. Let $b(\x)$ be a trial distribution with factor and variable marginals given by $\bn=\{\b_j\}_{j=1}^M$ and $\bv=\{b_i\}_{i=1}^N$. Then, the Bethe free energy $F_B(b)$ corresponding to the true distribution $p(x)$ is defined as
\begin{align}
F_B(b)&=F_B\left( \bn, \bv \right)=U_B(\bn, \bv) - H_B(\bn, \bv),  \label{eq_bfe_eg}
\end{align}
\vspace{-5mm}
\begin{align}
\text{where } U_B(\bn, \bv)=-\sum\limits_{j=1}^M \sum\limits_{{\x^{(j)}} \in S^{N_j}}  \b_j(\x^{(j)}) \ln f_j(\x^{(j)}). \label{eq_ub}
\end{align}
\end{definition}
 \subsubsection{Bethe optimization (BO)}
The following optimization problem is referred to as the Bethe optimization.
\begin{align}
&\underset{\bn, \bv} {\arg \min}\; \;  F_B(\bn, \bv), \text{  subject to}  \label{eq_bethe_min}\\
 b_i(x_i) &\geq 0, \hspace{0.4cm} i = 1, \dots, N, \; \;  x_i \in S,\nonumber\\ 
  \sum_{x_i} b_{i} (x_i)&=1, \hspace{0.4cm} i = 1, \dots, N, \nonumber\\ 
\b_j(\x^{(j)}) &\geq 0, \hspace{0.4cm} j = 1, \dots, M, \; \;   \x^{(j)} \in S^{N_j},\nonumber\\
 \sum_{\x^{(j)}} \b_{j} (\x^{(j)})&=1, \hspace{0.4cm} j = 1, \dots, M, \nonumber\\
 \sum_{\x^{(j)} \setminus \{x_i \}} \b_j(\x^{(j)})&= b_i(x_i), \hspace{0.2cm} j=1, \dots, M, \; i \in \N_j,\; x_i \in S ,\nonumber
\end{align}
where $\N_j$ is the set of indices of all the variable nodes associated with the factor node $j$.

\emph{Note:}
A feasible collection $(\bn,\bv)$ of the Bethe optimization problem does not necessarily represent the marginals of any coherent joint distribution over $S^N$, and are therefore referred to as \emph{pseudo-marginals} \cite{yedidia}. In spite of performing the optimization over a relaxed set, the solution of the Bethe optimization $(\bn^*, \bv^*)$ exactly coincides with the marginals of the true distribution $(\pn^*, \pv^*)$, if the underlying factor graph is a tree. Further, for factor graphs with loops, the solution leads to very good estimates of the true marginals \cite{yedidia, bethe_emprical}. In many applications, solving for the global minimizer of \eqref{eq_bethe_min} is not feasible because of its non-convexity. Hence, a stationary point of the BFE satisfying the constraints in \eqref{eq_bethe_min} is considered as a good estimate of the true marginals \cite{yedidia, bethe_emprical}.


\subsection{Bethe approximation for CSMA}
We observe that the stationary distribution of the CSMA Markov chain $p(\x)$ given by \eqref{eq_succint} is in product form \eqref{eq_factors} with the factor functions $\{f_j \}_{ j=1}^N$ defined as
\begin{align}
f_j(\x^{(j)})= \begin{cases}
\lambda_j, & \text{if }  x_j=1, \gamma_j(\x^{(j)}) \geq T, \label{eq_local_factors} \\
  0, & \text{if } x_j=1, \gamma_j(\x^{(j)}) < T, \\
 1,  & \text{if } x_j = 0.
\end{cases}
\end{align}
where $\x^{(j)}$ is the local schedule of the link $j$ defined earlier.

\begin{comment}
 Using these factor functions, $p(\x)$ can be equivalently represented as
\begin{align}
p(\x)&= \frac{1}{Z}\prod\limits_{j=1}^N f_j(\x^{(j)}),  \hspace{0.7cm} \x \in \{0,1\}^\N. \label{eq_dist_prod1}
\end{align}

Next, let us consider the factor graph representation of $p(\x)$. Observe that in $p(\x)$, the number of factor functions are equal to the number of variables nodes $N$, \ie, corresponding to each variable node $j$, there is a factor node $f_j$. For example, if we consider a network with the interference graph (defined in Section \ref{sec_model}) given by Figure \ref{fig_randomgraph}, then the corresponding factor graph is given by Figure \ref{fig_fg_sinr}. 
\end{comment}

By the definition of local feasibility, $p(\x)$ assigns zero probability to a schedule $\x$, if it is locally infeasible at any link. Hence, the factor node marginals $\pn = \{\p_j\}_{j=1}^N$ have to satisfy $\p_j(y)=0, \; \; \; \forall y \notin \I_j, \;  \forall j \in \N.$

\begin{comment}
If we recall the definition of local feasibility, it can be observed that the distribution $p(\x)$ assigns zero probability to a schedule $\x$, if it is locally infeasible at any link $j \in \N$. Hence, the factor node marginals $\pn = \{\p_j\}_{i=1}^N$ have to satisfy  
\begin{align}
\p_j(y)&=0, \; \; \; \forall y \notin \I_j, \;  \forall j \in \N. \label{eq_local_feasibility}
\end{align}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
       \begin{tikzpicture}[scale=0.2]
%\draw (0,0) -- (-2,0.7);
%\draw (-2,-0.7) -- (0,0);
%\draw (1.65,3.65) -- (2.35,3.65);
%\draw (1.65,4.35) -- (2.35,4.35);
%\draw (1.65,3.65) -- (1.65,4.35);
%\draw (2.35,3.65) -- (2.35,4.35);
%\node at (1.0,4) {{$f_{23}$}};
%
%\draw (4-.35,4.5-.35) -- (4+.35,4.5-.35);
%\draw (4-.35,4.5+.35) -- (4+.35,4.5+.35);
%\draw (4-.35,4.5-.35) -- (4-.35,4.5+.35);
%\draw (4+.35,4.5-.35) -- (4+.35,4.5+.35);
%\node at (4,5.5) {{$f_{35}$}};
%
%
%\draw (4-.35,2.5-.35) -- (4+.35,2.5-.35);
%\draw (4-.35,2.5+.35) -- (4+.35,2.5+.35);
%\draw (4-.35,2.5-.35) -- (4-.35,2.5+.35);
%\draw (4+.35,2.5-.35) -- (4+.35,2.5+.35);
%\node at (4,1.5) {{$f_{25}$}};
%
%
%\draw (8-.35,5.5-.35) -- (8+.35,5.5-.35);
%\draw (8-.35,5.5+.35) -- (8+.35,5.5+.35);
%\draw (8-.35,5.5-.35) -- (8-.35,5.5+.35);
%\draw (8+.35,5.5-.35) -- (8+.35,5.5+.35);
%\node at (8,6.5) {{$f_{15}$}};
%
%
%\draw (8-.35,1.5-.35) -- (8+.35,1.5-.35);
%\draw (8-.35,1.5+.35) -- (8+.35,1.5+.35);
%\draw (8-.35,1.5-.35) -- (8-.35,1.5+.35);
%\draw (8+.35,1.5-.35) -- (8+.35,1.5+.35);
%\node at (8,0.5) {{$f_{45}$}};


\draw (2,2)circle(0.4cm);
\node at (1.2,0.9) {{$2$}};
\draw (2,6)circle(0.4cm);
\node at (1.3,7) {{$3$}};
\draw (6,3)circle(0.4cm);
\node at (6.1,4.4) {{$5$}};
\draw (10,8)circle(0.4cm);
\node at (10.7,9) {{$1$}};
\draw (10,-0)circle(0.4cm);
\node at (10.8,-0.7) {{$4$}};
%\node at (3,0.85+0.2) {$2$};



\draw (6+0.2,3-0.2) -- (10-0.2,0+0.35); %3-5
%\draw (10-0.2,0+0.35) -- (8+.35,1.5-.35); %3-5

\draw (10-0.2,8-0.2) -- (6+0.2,3+0.2); %4-3
%\draw (6+0.2,3+0.2) -- (8-.35,5.5-.35); %3-4

\draw (6-0.2,3-0.2) -- (2+0.2,2+0.2); %3-1
%\draw (2+0.2,2+0.2) -- (4-.35,2.5-0); %1-3

\draw (6-0.2,3+0.2) -- (2+0.2,6-0.2); %3-1
%\draw (2+0.2,6-0.2) -- (4-.35,4.5+.35); %1-3

\draw (2,2+0.4) -- (2,6-0.4); %3-1
%\draw (2,6-0.4) -- (2,4+.35); %1-3
\end{tikzpicture}
\caption{interference graph}
\label{fig_randomgraph}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
       \begin{tikzpicture}[scale=0.3]
\draw (-1.5,3)circle(0.4cm);
\node at (-1.5,4) {{$x_2$}};

\draw (0.5,3)circle(0.4cm);
\node at (0.5,4) {{$x_3$}};

\draw (2.5,3)circle(0.4cm);
\node at (2.5,4) {{$x_5$}};
\draw (4.5,3)circle(0.4cm);
\node at (4.5,4) {{$x_1$}};
\draw (6.5,3)circle(0.4cm);
\node at (6.5,4) {{$x_4$}};
%\node at (3,0.85+0.2) {$2$};

\draw (-1.5-.35,0-.35) -- (-1.5+.35,0-.35);
\draw (-1.5-.35,0+.35) -- (-1.5+.35,0+.35);
\draw (-1.5-.35,0-.35) -- (-1.5-.35,0+.35);
\draw (-1.5+.35,0-.35) -- (-1.5+.35,0+.35);
\node at (-1.5,-1) {{$f_{2}$}};

\draw (0.5-.35,0-.35) -- (.5+.35,0-.35);
\draw (0.5-.35,0+.35) -- (.5+.35,0+.35);
\draw (0.5-.35,0-.35) -- (.5-.35,0+.35);
\draw (0.5+.35,0-.35) -- (.5+.35,0+.35);
\node at (.5,-1) {{$f_{3}$}};

\draw (2.5-.35,0-.35) -- (2.5+.35,0-.35);
\draw (2.5-.35,0+.35) -- (2.5+.35,0+.35);
\draw (2.5-.35,0-.35) -- (2.5-.35,0+.35);
\draw (2.5+.35,0-.35) -- (2.5+.35,0+.35);
\node at (2.5,-1) {{$f_{5}$}};

\draw (4.5-.35,0-.35) -- (4.5+.35,0-.35);
\draw (4.5-.35,0+.35) -- (4.5+.35,0+.35);
\draw (4.5-.35,0-.35) -- (4.5-.35,0+.35);
\draw (4.5+.35,0-.35) -- (4.5+.35,0+.35);
\node at (4.5,-1) {{$f_{1}$}};

\draw (6.5-.35,0-.35) -- (6.5+.35,0-.35);
\draw (6.5-.35,0+.35) -- (6.5+.35,0+.35);
\draw (6.5-.35,0-.35) -- (6.5-.35,0+.35);
\draw (6.5+.35,0-.35) -- (6.5+.35,0+.35);
\node at (6.5,-1) {{$f_{4}$}};



\draw (-1.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (0.5,0.35) -- (0.5,3-0.4); %B- x2
\draw (2.5,0.35) -- (2.5,3-0.4); %B- x2
\draw (4.5,0.35) -- (4.5,3-0.4); %B- x2
\draw (6.5,0.35) -- (6.5,3-0.4); %B- x2

%for node 2
\draw (-1.5,0.35) -- (0.5,3-0.4); %A- x1
\draw (-1.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 2
\draw (0.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (0.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 5
\draw (2.5,0.35) -- (0.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (4.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (6.5,3-0.4); %A- x1

%for node 1
\draw (4.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 4
\draw (6.5,0.35) -- (2.5,3-0.4); %A- x1

\end{tikzpicture}
\caption{Factor graph}
\label{fig_fg_sinr}
    \end{subfigure}
    \caption{Graphs associated with the SINR model}
\end{figure}
\end{comment}
\textbf{BFE for CSMA:}
We shall consider the product form representation of the CSMA stationary distribution $p(\x)$ in \eqref{eq_succint} and compute the BFE. As defined in \eqref{eq_bfe_eg}, the BFE for a given trial distribution $b(\x)$ has two terms $U_B(\bn,\bv)$, $H_B(\bn, \bv)$. Now we compute the first term $U_B(\bn, \bv)$. Specifically, we show that the term $U_B(\bn, \bv)$ which is in general a function of the factor marginals $\bn$, reduces to a function of just the variable marginals $\bv$, subject to the feasibility conditions stated in the following lemma.
\begin{lemma} \label{lemma_u_bethe}
Let $(\bn,\bv)$ be a set of feasible factor and variable marginals of the Bethe optimization problem \eqref{eq_bethe_min}.  If the factor marginals of a trial distribution $\bn$, assign zero probabilities to all the infeasible local schedules, \ie, 
 \begin{align}
 \b_j(y)=0, \;  \forall y \notin \I_j, \;  \forall j \in \N, \label{eq_bn_feasible}
 \end{align}
then $U_B(\bn, \bv)$ reduces to $U_B(\bn, \bv)=$ $U_B(\bv)= -\sum_{i=1}^N b_i(1) \ln\lambda_i.$ Moreover, if $\bn$ does not satisfy \eqref{eq_bn_feasible}, $U_B(\bn, \bv)=  \infty$, which in turn implies $F_B(\bn, \bv)=\infty$.
\end{lemma}
\begin{proof} %Proof is provided in Section IV of the supplementary material.
%\begin{comment}
Recalling the definition of local feasibility (introduced in Section \ref{local_gibbs}), we obtain
\begin{align*}
\I_j=\{\x^{(j)}\;|\; x_j = 0\} \cup  \{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) \geq T \}.
\end{align*}
Consider the inner summation of $U_B(\bn,\bv)$ in \eqref{eq_ub}, and expand it into two terms as follows:
\begin{align}
&\sum\limits_{\x^{(j)} \in \{0,1\}^{\N_j}} \b_j(\x^{(j)})  \ln f_j(\x^{(j)}) \nonumber\\
&=\sum\limits_{ \{\x^{(j)} \in \I_j \} } \b_j(\x^{(j)}) \ln f_j(\x^{(j)}) +\sum\limits_{\{\x^{(j)} \notin \I_j \}} \b_j(\x^{(j)}) \ln f_j(\x^{(j)}). \label{eq_summation}
\end{align}
Now, we evaluate the first term of \eqref{eq_summation}.

\vspace{-4mm}
\begin{scriptsize}
\begin{align}
&\sum\limits_{ \{\x^{(j)} \in \I_j \} } \b_j(\x^{(j)}) \ln f_j(\x^{(j)}) \overset{(a)}{=} \nonumber \\
&\sum\limits_{\{\x^{(j)}\;|\; x_j = 0\}} \b_j(\x^{(j)}) \ln f_j(\x^{(j)}) +\sum\limits_{\{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) \geq T \}} \b_j(\x^{(j)}) \ln f_j(\x^{(j)})   \nonumber, \\
&\overset{(b)}{=}\sum\limits_{\{\x^{(j)}\;|\; x_j = 0\}} \b_j(\x^{(j)}) \ln 1 + \sum\limits_{\{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) \geq T \}} \b_j(\x^{(j)}) \ln \lambda_j  \nonumber,  \\
&=\ln \lambda_j \sum\limits_{\{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) \geq T \}} \b_j(\x^{(j)}).\label{eq_lemma_ub1}
\end{align}
\end{scriptsize}
\vspace{-4mm}

where $(a)$ follows from the definition of local feasibility, $(b)$ follows from the defintion of factors in \eqref{eq_local_factors}.

We now show that the second term of \eqref{eq_summation} evaluates to zero. If $\x^{(j)} \notin \I_j$, then from \eqref{eq_local_factors} and the assumption \eqref{eq_bn_feasible}, we have $f_j(\x^{(j)})=0$ and $\b_j(\x^{(j)})=0$ respectively. Hence the summation corresponding to ${\{\x^{(j)} \notin \I_j \}}$ in \eqref{eq_summation} is equal to zero.


Now, we use the fact that $(\bn,\bv)$ is feasible for the Bethe optimization problem \eqref{eq_bethe_min}. Specifically, we use the last equality constraint in \eqref{eq_bethe_min} for $i=j$ case (recall from the definition of $\N_j$, that the link $j$ is also included in the set $\N_j$) to obtain

\vspace{-3mm}
\begin{scriptsize}
\begin{align}
&b_j(1)=\sum\limits_{\{\x^{(j)}\;|\; x_j=1\}} \b_j(\x^{(j)}), \nonumber \\
&=\sum\limits_{\{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) \geq T \}} \b_j(\x^{(j)}) + \sum\limits_{\{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) < T \}} \b_j(\x^{(j)}), \nonumber \\
&\overset{\eqref{eq_bn_feasible}}{=}\sum\limits_{\{\x^{(j)}\;|\; x_j=1, \gamma_j(\x^{(j)}) \geq T \}} \b_j(\x^{(j)}) + 0. \label{eq_lemma_ub2}
\end{align}
\end{scriptsize}
\vspace{-3mm}

Substituting  \eqref{eq_lemma_ub1}, \eqref{eq_lemma_ub2} in \eqref{eq_summation}, we obtain
\begin{align*}
\sum\limits_{\x^{(j)} \in \{0,1\}^{\N_j}} \b_j(\x^{(j)})  \ln f_j(\x^{(j)}) = b_j(1) \ln \lambda_j .
\end{align*}
Using the above equation in the definition of $U_B(\bn,\bv)$ in \eqref{eq_ub} completes the proof of this Lemma.
%\end{comment}
\end{proof}
%\begin{align*}
%U(b)&= -\sum\limits_{\ds \in \{0,1\}^\N} b(\ds) E(\ds), \\
%&=-\sum\limits_{\ds \in \{0,1\}^\N} b(\ds) .\left(-\sum\limits_{a=1}^N \mu_a \left( \ds(\bar{\N_a}) \right)\log(\lambda_a)\right),  \\
%&=-\sum\limits_{a=1}^N \left(\sum\limits_{\dnaa \in \{0,1\}^{\naa}} \mu_a\left( \dnaa \right)b_{\naa}\left(\dnaa\right) \right)\log(\lambda_a),\\
%&= -\sum\limits_{a=1}^N \log(\lambda_a) \E_{b_{\naa}}[\mu_a], \\
%&= -\sum\limits_{a=1}^N \log(\lambda_a) b_a(1).
%\end{align*}
Using Lemma \ref{lemma_u_bethe} and \eqref{eq_bfe_eg}, the BFE for any $(\bn, \bv)$ that satisfies the feasibility constraints in \eqref{eq_bethe_min}, \eqref{eq_bn_feasible} is given by
\begin{align}
F_B(\bn,\bv)&=F_B\left( \{\b_j\}_{j=1}^N,  \{b_i\}_{i=1}^N \right),  \label{eq_bfe}\\
&= \sum\limits_{i=1}^N  -b_i(1) \ln\lambda_i  - \H_i(\b_i)  +  (d_i-1) H_i(b_i), \nonumber
\end{align}
where $d_i$ is degree of variable node $i$ in the factor graph. We refer $F_B(\bn,\bv)$ \eqref{eq_bfe} as the BFE corresponding to the set of fugacities $\{\lambda_i\}_{i=1}^N$. It essentially means that $F_B(\bn,\bv)$ is the BFE corresponding to $p(\x)$ in \eqref{eq_succint}. 

\emph{Remark:}  Since we are only interested in the Bethe optimization problem \eqref{eq_bethe_min}, throughout this paper, we implicitly assume that the factor and variable marginals $(\bn,\bv)$ satisfy the feasibility conditions in \eqref{eq_bethe_min}, \eqref{eq_bn_feasible}, and use the BFE $F_B(\bn,\bv)$ expression obtained in \eqref{eq_bfe}.

%This is because, for any $(\bn, \bv)$ that does not satisfy \eqref{eq_bn_feasible}, $F_B(\bn, \bv) = \infty$. Hence, such $(\bn, \bv)$ cannot be optimal point of \eqref{eq_bethe_min}.



%{\color{blue} Before we proceed to our main results, let us make some remarks on the terminology that will be used in the results.
%\begin{itemize}
%\item  From \eqref{eq_bfe}, it can be observed that a set of fugacities $\{\lambda_i\}_{i=1}^N$ define the BFE corresponding to CSMA distribution $p(x)$ in \eqref{eq_succint}. Hence, \eqref{eq_bfe} will be referred to as the BFE corresponding to the set of fugacities $\{\lambda_i\}_{i=1}^N$.
%\item As discussed earlier, a stationary point $(\bn^*, \bv^*)$ of the BFE \eqref{eq_bfe} corresponds to approximate marginals of the true distribution $p(x)$. In particular, in the context of CSMA, the variable marginals $\bv^*=\{b_j^*(1)\}_{j=1}^N$ are nothing but the approximate service rates corresponding to the fugacities $\{\lambda_j\}_{j=1}^N$. 
%%Hence, the service rates will be referred to as the variable marginals at the stationary point of the BFE.
%%In this spirit, we will use statements like ``A set of service rates $\{s_i\}_{i=1}^N$ is a stationary point of the BFE corresponding to the set of fugacities $\{\lambda_j\}_{j=1}^N$".
%\end{itemize}}




==> ArXiv Version TON/special_cases_1.tex <==
Conflict graph model \cite{bethe_jshin} is a special case of the SINR interference model. In the conflict graph model, two links cannot transmit simultaneously, if one link is within the interference range of the other link. Under the conflict graph model, we derive simple closed form expressions for the local fugacities  \eqref{opt_local_alternate0}.
%In this section, we consider the conflict graph model \cite{bethe_jshin} which is a of the special case of the SINR interference model. We derive simple closed form expressions for the local fugacities, which are otherwise to be obtained by solving the optimization problem \eqref{opt_local_alternate0}.
%In the conflict graph model, two links cannot transmit simultaneously if one link is within the interference range of the other link. The set of local feasible schedules $\I_i$ has only one feasible local schedule with link $i$ being active (\ie, the local schedule with just link $i$ being active and all the neighbors inactive). In all other feasible local schedules the link $i$ is inactive. By taking advantage of this simple structure of $\I_i$, the local fugacities are derived as follows.
\begin{theorem} \label{thm_lf_cg}
 For the conflict graph model, the local fugacities \ie, solution of the local Gibbsian problem \eqref{opt_local_alternate0} at a link $i$ is given by
\begin{align}
e^{\lf_{ij}}&= \begin{cases} \label{eq_lf_cg}
s_i  \left(1-s_i\right)^{|\N_i|-2} \prod\limits_{k \in \N_i \setminus \{i\}}(1-s_i-s_k)^{-1},\; \text{if } j=i, \\
s_j(1-s_i-s_j)^{-1}, \; \; \; \; \; \text{if } j \in \N_i \setminus \{i\}.
\end{cases}
\end{align}
\end{theorem}
\begin{proof}
Proof is provided in Appendix \ref{proof_lf_cg}. %X-D of the supplementary material. %
\end{proof}
\noindent \emph{Comparison with the results in \cite{bethe_jshin}:}\\
The fugacities for the conflict graph model have been derived in \cite{bethe_jshin}. Here, we derive the global fugacities using our approach and compare to the results in \cite{bethe_jshin}. 
%To that end, we derive the global fugacities using our approach proposed in this paper.
\begin{cor}
 \label{cor_cg}
 For the conflict graph model, the global fugacity at a link $i$ is
\begin{align*}
\tilde{\lambda}_i&= \frac{s_i (1-s_i)^{2|\N_i|-3}}{\prod\limits_{k \in \N_i \setminus \{i\}} (1-s_i-s_k)^2}.
\end{align*}
\end{cor}
\begin{proof}
We obtain this result by substituting the local fugacities obtained in \eqref{eq_lf_cg} in the expression proposed for global fugacities \eqref{eq_lf_gf0}.
\end{proof}
The expression for the global fugacities proposed in \cite{bethe_jshin} is
\begin{align*}
\tilde{\lambda}_i&= \frac{s_i (1-s_i)^{|\N_i|-2}}{\prod\limits_{k \in \N_i \setminus \{i\}} (1-s_i-s_k)},
\end{align*}
which is different from the expression derived in Corollary \ref{cor_cg}. In essence, these expressions are different because, the factorizations considered in the two cases are different. Specifically, it is well known that for a given product form distribution, the Bethe approximation technique could lead to different results, corresponding to different factorizations of the product form distribution \cite[Chapter 2, Page 10]{book_martin}.

% well known fact that 
%
%It looks a bit surprising because, both these expressions are derived for the same conflict graph model using the Bethe approximation techniques. This surprising behaviour can be explained using the following facts: a) A product form distribution can be factorized in multiple ways. b) For the same product form distribution, the Bethe approximation technique could lead to different results if the underlying factorization of the product form distribution is different \cite{yedidia}.

To elucidate this point, we consider the conflict graph interference model, and present two natural factorizations that lead to the same CSMA distribution  \eqref{eq_dist}. 
%
%Let $G(V,E)$ be the conflict graph used to model the interference. Then CSMA product form distribution is given by
%\begin{align*}
%p(\x)&= \frac{1}{Z} \prod_{j \in V} \lambda_j^{x_j} \i(\x \text{ is feasible}), \; \; \x \in \{0,1\}^{\N}
%\end{align*}
In the conflict graph model, a schedule $\x$ is said to be feasible if it is an independent set of the underlying graph $G(V,E)$. Using this observation, the term $\i(\x \text{ is feasible})$ in \eqref{eq_dist} can be factorized in two ways as given below.\\
\emph{1. Edge-centric factorization:} This factorization ensures that for each edge, not more than one of its end vertices are active.
\begin{align*}
\i(\x \text{ is feasible})&= \prod_{(i,j) \in E} \i(x_i x_j =0).
\end{align*}


\noindent \emph{2. Vertex-centric factorization:} In this factorization, whenever a vertex is active, it ensures that all its neighbours are inactive.
\begin{align*}
\i(\x \text{ is feasible})&= \prod_{j \in V} f_j({\x^{(j)}}),
\end{align*}
where $\x^{(j)}$ is the set of activation status of node $j$ and its neighbours, and $f_j$ is given by
\begin{align*}
f_j(\x^{(j)})= \begin{cases}
 1,  & \text{if } x_j = 0,\\
1, & \text{if }  x_j=1 \text{ and } \{x_k\}_{k \in \N_j \setminus \{j\}}=0, \\
  0, &  \text{otherwise}.
\end{cases}
\end{align*}
In \cite{bethe_jshin}, the authors use the edge-centric factorization, which cannot be directly used to capture the SINR model. Hence we use a more general factorization \eqref{eq_local_factors}, which reduces to the vertex-centric factorization for the conflict graph case. 

\emph{Remark:} 
The existing theory on the Bethe approximation is not sufficient to conclude or prove that one of the factorizations is always better than the other. However, the following can be said under some special cases.

\begin{itemize}
\item For the conflict graph model, the formula derived in \cite{bethe_jshin} is provably exact if the conflict graph is a tree. Hence, if there is prior knowledge that the conflict graph has tree topology, the formula in \cite{bethe_jshin} should be used. 

\item From the simulations that we have conducted, we have the following observation for topologies with loops. For the formula proposed in \cite{bethe_jshin}, we observed that the achieved service rate is less than the target service rate even for small load. However, for the formula obtained using our approach, the achieved service rate is more than the target service rate at smaller loads. Hence, if we have prior knowledge that we are operating in the low load regime, empirical evidence suggests that it is beneficial to use the approach proposed in our paper.
\end{itemize}

%However, 
 %while In our work, we have used the vertex-centric approach (as the egde-centric approach is not applicable for the general SINR based interference model). While both these approaches deal with the same distribution $p(\x)$ in \eqref{eq_dist}, the factors are chosen differently. Hence, because of this difference in the choice of factorization, the Bethe approximation could lead to different results despite the fact that they consider the same distribution.

 %If one is interested only in the conflict graph interference model, it is recommended to use the edge-centric model as it exploits the structure of the conflict graph model to give a simple pair-wise interaction model.


%Let us consider a simple 4-cycle as our conflict graph. Let the vertices and edges be given as $V=\{1,2,3,4\}$, $E=\{(1,2), (2,3), (3,4), (4,1)\}$. Then the product form distribution on the feasible schedules can be written as
%\begin{align*}
%p(\x)&= \frac{1}{Z} \prod_{j \in V} \lambda_j^{x_j} \prod_{(i,j) \in E} \i(x_i x_j =0), \; \;  \x \in \{0,1\}^4.\, \\
%p(\x)&= \frac{1}{Z} \prod_{j \in V} \lambda_j^{x_j} \prod_{j \in V} f_j({\x^{(j)}}) ,\; \;  \x \in \{0,1\}^4.
%\end{align*}
%where the second factorization is over the local schedules. For example, the factor $f_2$ which is a function of $\x^{(2)}=\{x_2,x_3,x_4\}$ is given by
%\begin{align*}
%f_2(x_2,x_3,x_4)= \begin{cases}
% 1,  & \text{if } x_2 = 0,\\
%1, & \text{if }  x_2=1, x_3=0 \text{ and } x_4=0,  \\
%  0, &  \text{otherwise}.
%\end{cases}
%\end{align*}

\begin{comment}
\subsection{Conservative SINR model}
In the conservative SINR model considered in \cite{sinr_mimo}, the neighboring links of a link $i$ are ranked in an ascending order based on the interference they incur to link $i$. Then, the set of neighboring links $\N_i$ is partitioned into two disjoint sets $\N^A_i$ and $\N^B_i$. The set $\N^A_i$ is obtained by adding the neighboring links one by one, starting from the link incurring the lowest interference to the highest, till the aggregate interference of all the links in $\N_i^A$ is small enough to maintain the required SINR threshold $T$ at link $i$. All the neighboring links which are not in  $\N^A_i$ are said to be intolerable and are included in the set $\N_i^B$. Let $d_i^a$, $d_i^b$ be the sizes of the sets. Then the local fugacities can be related to the service rates as follows.
\begin{theorem} \label{thm_lf_cs}
For the conservative SINR model, the local fugacities have the following closed form expressions:
\begin{align}
e^{\lf_{ij}}&= \begin{cases} \label{eq_lf_cs}
s_i  \left(1-s_i\right)^{d_i^b-1} \prod\limits_{k \in \N_i^B}(1-s_i-s_k)^{-1},& \text{if } j=i, \\ 
s_j(1-s_i-s_j)^{-1}, & \hspace{-1cm} \text{if } j \in \N_i^B, \\
s_j(1-s_j)^{-1},& \hspace{-1cm} \text{if } j \in \N_i^A. 
\end{cases} 
\end{align}
\end{theorem}
\begin{proof}
Proof is provided in Appendix \ref{proof_lf_cs}.
\end{proof}
\end{comment}



==> ArXiv Version TON/system_model.tex <==
We consider a single-hop wireless network and model the links using a bipole model, introduced in \cite{baccelli}. In a bipole model, each transmitter is associated with a receiver on the Euclidean plane.  A transmitter and its corresponding receiver are referred to as a link. Let $\N$ denote the set of all the links in the network. Let $|\N| =N$ be the total number of links. Let $r_{ii}$ denote the distance between the transmitter and receiver of link $i$. For simplicity, we assume\footnote{The results in this paper do not require this assumption. This is just to keep the expressions concise.} that a link distance $r_{ii}$ is much smaller than the distances of the transmitter and the receiver from the other links.  With this assumption, we can think of links as points in the Euclidean space $\R^2$. Let $r_{ji}$ denote the distance between the links $i, j$. We assume a time slotted model.

\emph{Interference model:}
We consider the standard path-loss model $\|d\|^{-\alpha}, \alpha>2$, where $d$ is the distance between a receiver and a transmitter, and $\alpha$ is the path loss exponent. Let $P_i$ denote the transmit power of link $i$. We assume white Gaussian thermal noise  at all the receivers with variance $w$. Let $\x(t)=[x_i(t)]_{i=1}^N$ denote the schedule of the network at time $t$. Specifically, $x_i(t)=1$ denotes that the link $i$ is active (transmitting) in time slot $t$. If there is no ambiguity, we will also use $\x$ to denote $\x(t)$.

  Although all the active links in the network can potentially contribute to the interference, the aggregate interference from the transmitters beyond a certain distance can be safely neglected \cite{radius_approx1}, \cite{radius_approx2}. This approximation is standard in the literature \cite{sinr_mimo} and this distance, referred to as the \emph{close-in} radius is denoted by $R_I$. Let $\N_i:= \lbrace k \; | \; r_{ik} \leq R_I \rbrace $. For convenience, let link $i$  be also included in the set $\N_i$. We refer to the links in $\N_i \setminus \{i\}$ as the neighbors of link $i$.  The neighborhood relationship can be represented by an \emph{interference graph} $G(V,E)$. $V$ is the set of links in the network and two links share an edge if they are within a distance $R_I$. Then the total interference power at link $i$ is given by
\begin{align}
I_i(\x) = \sum\limits_{ \{ j \in \N_i \;|\; j \neq i,\; x_j=1\}} P_j r_{ji}^{-\alpha}. \label{eq_int1}
\end{align}
Then, the SINR at link $i$ is given by
\begin{align}
\gamma_{i}(\x) =\frac{P_i r_{ii}^{-\alpha}}{I_i(\x)+w}. \label{eq_sinr}
\end{align}
% Here, $P_i r_{ii}^{-\alpha}$ is the received power at the receiver of link $i$  from its intended transmitter, and $w$ is the thermal noise power.
 
\emph{Reception model:}
We assume that, in each time slot, a single packet of data is transmitted from each active transmitter. If the received SINR at the corresponding receiver exceeds a pre-determined threshold T, \ie, $\gamma_i(\x) \geq T$, the packet is successfully received.

 % \begin{comment}
%Let $\N_i^T$ denote the set of links whose transmitters are potential interferers of the receiver of link $i$ (\ie, the set of transmitters within the ball of radius $R_I$ around the receiver of link $i$). 
%\begin{align*}
%\N_i^T:= \lbrace \; k \; | \; k \neq i, r_{ik} \leq R_I \rbrace.
%\end{align*}
%Similarly, let $\N_i^R$ denote the set of receivers for which the transmitter of link $i$ is one of the potential interferers. 
%\begin{align*}
%\N_i^R:= \lbrace \; k \; | \; k \neq i, r_{ki} \leq R_I \rbrace.
%\end{align*}
% 
%Thus \eqref{eq_sinr} can be written as,
%\begin{align}
%\gamma_{i}(\ds) =\frac{PR^{-\alpha}}{I\left(\M^T_i \setminus\lbrace i \rbrace\right)+w}, \label{eq_sinr1}
%\end{align}
%where, $\M_i^T \subset \N_i^T$ denotes the set of potential interferers of link $i$ that are active in the schedule $\ds$. 
% 
%
%
%Two links $i,j$ are said to be \emph{dependent} if atleast one of the following two conditions are met.
%\begin{itemize}
%\item[i)] Link $i$ is a potential interferer of $j$ 
%\item[ii)] Link $j$ is a potential interferer of link $i$.
%\end{itemize}
%
%Let 
%Hence, the set of links, with which link $i$ is dependent are $ \N_i^T \cup \N_i^R$. This dependency can be modelled by an undirected graph $G(V,E)$ with $V=\N$ in which, two links are connected by an edge if they are dependent. This graph only captures the dependency relation. However to fully capture the interference constraints, we augment the dependency graph with a set of vectors called  \emph{self tolerance} vectors. 
%
%
%\begin{align}
%\N_i^D=
%\end{align}
%
%\begin{definition} Two links $i,j$ are said to be \emph{dependent} if either $j \in \N_i^T$ or $j \in \N_i^R$.
%\end{definition}
%The links in $\N_i$ are referred as the neighbours of link $i$. Thus, from \eqref{productform} the probability of success is,
%\end{comment}
\emph{Rate region:}
\begin{comment}
For a conflict graph based interference model, a feasible schedule is defined as follows.
\begin{definition}
A schedule $\ds$ is said to be \emph{feasible} in the conflict graph model, if no two interfering links are active in the schedule, \ie,
\begin{align*}
\ds_i+\ds_j &\leq 1, & \forall  (i,j) \in E.
\end{align*}
\end{definition}
The set of all the feasible schedules for the conflict graph model is denoted by $\mathcal{I}_C$.


Here, we define a notion of the feasible schedule for the SINR model, which overcomes the limitations of the conflict graph based interference model.

\end{comment}
A schedule $\x \in \{0,1\}^{\N}$ is said to be \emph{feasible}, if all the active links in the schedule meet the required SINR constraint, \ie , $\gamma_i(\x) \geq T, \; \forall i \text{ such that } x_i =1.$ The set of all the feasible schedules is denoted by $\mathcal{I}$. In our scenario, since each link transmits one data packet whenever it is successful, the long-term service rate of a link is equal to the fraction of time the link is successful. The \emph{rate region} $\Lambda$, which is defined as the set of all the possible service rates is given by the convex hull of the feasible schedules in $\mathcal{I}$.  Hence, $\Lambda= \{ \sum_{ \x \in \mathcal{I}} \alpha_{\x} \x \; | \; \sum_{\x \in \mathcal{I}} \alpha_{\x}=1, \; \alpha_{\x} \geq 0, \; \x \in \mathcal{I} \}$. If a link scheduling policy can support any rate vector in the rate region, then the scheduling policy is said to be \emph{rate-optimal}. 

\emph{Adaptive CSMA:} 
\label{subsec_acsma}
We briefly review the adaptive CSMA algorithm \cite{libin, sinr_mimo_journal}. In this algorithm, each link $i$ is associated with a fugacity $\lambda_i > 0$ which defines the underlying Gibbs distribution. In each time slot, a randomly selected link $i$ is allowed to update its schedule $x_i(t)$ based on the information in the previous slot:
\begin{itemize}
\item If its SINR is inadequate, \ie,  $\gamma_i(\x(t-1)) \leq T$, then $x_i(t)=0$.
\item If $\gamma_i(\x(t-1)) \geq T$, then link $i$ exchanges control messages with its neighbors, to find if they can meet their SINR requirements if link $i$ gets activated. If any of its neighbors cannot meet its requirement, then $x_i(t)=0$.
\item If all the neighbors can meet their SINR requirements even if link $i$ gets activated, then $x_i(t)=1$ with probability $\frac{\lambda_i}{1+\lambda_i}$, and $x_i(t)=0$ with probability $\frac{1}{1+\lambda_i}$.
\end{itemize}
\emph{Remarks on Implementation:}  A challenge in the second step of the above algorithm is to ensure that a newly scheduled link does not alter the SINR requirements of its transmitting neighbours. This problem is typically addressed by introducing a control subslot during which nodes exchange control packets to determine the feasibility of transmissions. More specifically, \cite{sinr_mimo_journal} proposed a control protocol which includes a three-way handshake of control packets: Ready-To-Send (RTS), Clear-To-Send (CTS), and REJECT. In this protocol, if a link is selected to update its status, its transmitter sends an RTS in the control subslot. If any active neighbouring link in the previous schedule $\x(t-1)$ fails to meet the required SINR, the neighbour broadcasts a REJECT signal and disapproves the transmission request. If no REJECT signal is broadcasted, the selected link proceeds to transmit. Detailed descriptions of this handshake protocol can found in \cite[Section III-C]{sinr_mimo_journal}.


It can be shown \cite[Proposition 1]{qcsma} that the adaptive CSMA algorithm induces a Markov chain on the state space of the schedules $\{0,1\}^\N$. Further, the stationary distribution of the Markov chain, parametrized by the fugacity vector $\lambda=[\lambda_i]_{i=1}^N$, is given by:
%\begin{align}
%p(\x) =\begin{cases}
%\frac{1}{Z} \prod\limits_{  j  : x_j=1}\lambda_j , & \forall \x \in \mathcal{I}, \label{eq_dist} \\
%0,&\forall \x \in \{0,1\}^{\N} \setminus \mathcal{I},
%\end{cases}
%\end{align}
\begin{align}
p(\x)&= \frac{1}{Z}\prod\limits_{  j \; : \; x_j=1}\lambda_j \; \i (\x \in \mathcal{I}) , & \forall \x \in \{0,1\}^N,  \label{eq_dist}
\end{align}
where $\i(\x \in \mathcal{I})$ is an indicator of $\x$ being a feasible schedule, and $Z$ is the normalizing constant. Then, due to the ergodicity of the Markov chain, the long-term service rate of a link $i$ denoted by $s_i$ is equal to the marginal probability that link $i$ is active, \ie, $p_i(x_i=1)$. Thus, the service rates and the fugacities are related as follows:
\begin{align}
s_i&= p_i(1) = \sum\limits_{\x \; : \; x_i=1 } Z^{-1} \prod\limits_{ j \; : \; x_j=1}\lambda_j, \; \; \forall i \in \N, \label{eq_serv_fug}
\end{align}
where $p_i(1)$ denotes $p_i(x_i=1)$.
The adaptive CSMA algorithm can support any service rate in the rate region provided appropriate fugacities are used for the underlying Gibbs distribution \cite[Theorem 5]{fast_mixing} . 

If the desired service rates are known, these fugacities can be obtained by solving the system of equations in \eqref{eq_serv_fug}.   In \cite[Section 3.3]{libin_book}, it is shown that solving this system of equations can be posed as a convex optimization problem. The main idea is explained as follows. Given a set of service rates from the rate region, by the definition of rate region, there should exist some distribution $\alpha(\x)$ on the state space of feasible schedules $\I$ which would support the required service rates. Note that the definition of rate region does not impose that the distribution $\alpha(\x)$ is a Gibbs distribution. In \cite[Section 3.3]{libin_book}, the authors find a Gibbs distribution that is close to this distribution $\alpha(\x)$. It is achieved by minimizing the KL divergence~\cite[Section 3.3]{libin_book} between $\alpha(\x)$ and the family of Gibbs distributions parameterized by the fugacity vectors. Further it has been shown \cite [Section 3.3]{libin_book} that the resulting minimization problem is equivalent to the following Gibbsian optimization problem referred to as the global problem.  

\noindent \textbf{The global Gibbsian problem:}
\begin{align}
\ln \lambda &= \arg\max_{r \in \R^{\N}} G(r), \label{opt_global} \\
\text{where  }G(r)&:=\sum\limits_{k \in \N} s_k r_{k} - \ln \Big(\sum\limits_{y \in \I} \exp\Big(\sum\limits_{k \in \N} y_k r_{k} \Big)\Big). \nonumber
\end{align} 
Here $\{s_i\}_{i \in \N} \in \Lambda$ are the desired service rates. 

 
\noindent \emph{Remark:}  To understand that the global Gibbsian problem \eqref{opt_global} solves the system of equations in \eqref{eq_serv_fug}, we can simply set  $\frac{\partial G(r)}{\partial r_i}=0$ to obtain
\begin{align*}
s_i - \frac{\sum_{y \in \I : y_i=1} \exp\Big(\sum_{k=1}^N y_k r^*_k\Big)}{\sum_{y \in \I} \exp\Big(\sum_{k=1}^N y_k r^*_k\Big)}=0, \; \forall i \in \N.
\end{align*}
Observe that for $\lambda_i= e^{r_i^*}$, the above equations essentially boil down to the desired equations in \eqref{eq_serv_fug}.


A distributed stochastic gradient descent algorithm was proposed in \cite{libin} to solve \eqref{opt_global}. However, estimating the gradient of $G(r)$ in a distributed manner entails the underlying Markov chain of the CSMA algorithm to converge to steady-state, which takes an impractically long time in general \cite{parallel_chains}. 

In the next section, we consider this scenario where the links know their target service rates. We provide an efficient and scalable approximation to this problem, by proposing the following local Gibbsian problems. The solutions of these local problems are appropriately combined to estimate the solution to the global problem.

==> ArXiv Version TON/umax.tex <==
In this section, we consider the utility maximization problem and provide an approximation algorithm to solve the problem in a distributed manner. The problem is defined as follows. Suppose each link $i$ in the network is associated with a concave utility function of its service rate $U_i : [0,1] \rightarrow \R_+$. Our objective is to find the service rates that maximize the system wide utility, \ie, 
\begin{align}
\max_{y \in \Lambda} \sum_{i=1}^N U_i(y_i), \label{eq_util_main}
\end{align}
and subsequently compute the global fugacities that correspond to these optimal service rates.

In \cite{libin}, an iterative algorithm to update the global fugacities is proposed. However, each iteration of the algorithm requires an underlying slowly mixing Markov chain to reach steady state. Hence it suffers from impractically slow convergence to the optimal fugacities. To address this issue, we propose an iterative algorithm which updates the local fugacities instead of directly updating the global fugacities. These local fugacitiy updates are computationally simple and do not require any Markov chain to convergence. These local fugacities are then used to obtain the approximate global fugacities using \eqref{eq_lf_gf0} proposed in Section \ref{local_gibbs}. 

Each link in the network executes \emph{Algorithm 2} in parallel. The algorithm involves solving an one dimensional optimization problem \eqref{eq_one_dim} related to the original optimization problem \eqref{eq_util_main}. Here $\theta >0,$ is a parameter of the algorithm that can be tuned. The solution of this optimization problem $s_j(t)$ is used in the subsequent steps of the algorithm to update the local fugacities \eqref{eq_update} and the global fugacities. We will later show that the update equation \eqref{eq_update} is inspired by a subgradient descent algorithm for a related optimization problem. The term $\alpha(t)$ in  \eqref{eq_update} corresponds to the step-size of the subgradient descent algorithm. Any standard step-sizes that satisfy the convergence criteria for a subgradient descent method can be used \cite[Chapter 2]{book_subgradient}. A typical example is $\alpha(t) = \frac{1}{t}$.

\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Algorithm 2: Local utility maximization at link $j$}\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
%\; \; \textbf{Input:} $\left( U_{k}(\cdot), \;  k \in \nj  \right)$; \hspace{0.25cm}
%\textbf{Output:} $\lt_j$%$\left(\lt_k, \;  k \in \N  \right)$.
\begin{enumerate}
\item At $t=0$, initialize $\beta_{jk}(t)=0,  \; \forall k \in \nj$.\\


\emph{Computing global fugacities:}\\

\item  From each neighbour $k \in \N_j$, obtain the local fugacity $\lf_{kj}(t)$. %Obtain the local fugacities $\left( \lf_{kj}(t), \; k \in \nj \right)$ from the neighbours.

\item Compute $s_j(t)$ as
\begin{align}
s_j(t)= \arg \max_{q \in [0,1]} \theta U_j(q) - q \sum_{k \in \nj} \beta_{kj}(t). \label{eq_one_dim}
\end{align}

\item Compute the approximate global fugacity $\lt_j(t)$ from local fugacities $\left( \lf_{kj}(t), \; k \in \nj \right)$ and $s_j(t)$ using \eqref{eq_lf_gf0}.\\
%\begin{align}
%\lt_j&= \left(\frac{1-s_j}{s_j}\right)^{|\N_j|-1}\prod\limits_{k \in \N_j} e^{\lf_{kj}}, \; \; \forall j \in \N. %\label{eq_lf_gf0}
%\end{align}

\emph{Updating the local fugacities:}\\
\item Consider the distribution
\begin{align*}
\b_j(\x^{(j)};t) =  {Z_j^{-1}} \exp \Big(\sum_{k \in \N_j} x_k \beta_{jk}(t) \Big),  \forall \x^{(j)} \in \I_j,
\end{align*}
  and for each $k \in \N_j$, let $m_{jk}(t):=\sum_{\x^{(j)} : x_k=1} \b_j(\x^{(j)};t)$ represent the marginal probability corresponding to $x_k$ under this distribution. 
\item For each $k \in \nj$, obtain $s_k(t)$ computed at the neighbour $k$, and update the local fugacity at $j$ using
\begin{align}
\beta_{jk}(t+1)= \beta_{jk}(t) + \alpha(t)\left(s_k(t)-m_{jk}(t)\right). \label{eq_update}
\end{align}
\end{enumerate}
\noindent\rule[0.5ex]{\linewidth}{0.5pt}

\emph{Complexity:}
The computational complexity of the above algorithm is $O(2^{|\N_j|})$, which depends only on the size of the local neighbourhood, and is independent of the total size of the network.
%The required information exchange and the complexity of the algorithm in an iteration, depend only on the size of the local neighbourhood, and is independent of the total size of the network.

\emph{Accuracy:}
The accuracy of the above algorithm can be understood by splitting the error into two parts. The first part is the error involved in estimating the optimal service rates in \eqref{eq_util_main}. The second part is the error involved in estimating the global fugacities corresponding to these service rates. We characterize the first part of the error in Theorem \ref{thm_util}, which states that the gap to the optimum utility is $O(\frac{1}{\theta})$.  In other words, the local algorithm provides a good estimate of the optimal service rates when $\theta$ is large. The second part of the error depends only on the accuracy of the Bethe approximation. The Bethe error is evidenced to be reasonably small in many applications \cite{bethe_emprical}.

 
\begin{theorem} \label{thm_util}
In Algorithm 2, the service rates $s(t)=[s_j(t)]_{j=1}^N$ \eqref{eq_one_dim} converge to some $\underline{s}=[\underline{s}_j]_{j=1}^N \in [0,1]^{\N}$, such that the limit $\underline{s}$ satisfies
\begin{align}
\sum_{j=1}^N U_j(\underline{s}_j) \geq \max_{y \in \Lambda} &\sum_{j=1}^N U_j(y_j) - \frac{\sum_j \log |\mathcal{I}_j|}{\theta}. \label{eq_thm_util}
\end{align}
\end{theorem}
\begin{proof}
We prove this theorem in the following steps:
\begin{itemize}
\item[1.] First, we define a new optimization problem \eqref{eq_util_bethe} that is related to the original utility maximization problem \eqref{eq_util_main}.
\item[2.] Then, we prove that the proposed local utility maximization algorithm corresponds to a subgradient descent algorithm for the new optimization problem \eqref{eq_util_bethe}.
\item[3.] Finally, we complete the proof by showing that the solution of the new optimization problem \eqref{eq_util_bethe} satisfies the inequality \eqref{eq_thm_util} stated in this theorem.
\end{itemize} 
\noindent  \emph{Step 1:}
Firstly, we relax the constraints of \eqref{eq_util_main} by replacing the actual capacity region $\Lambda$, with the Bethe approximated capacity region defined below:
\begin{align}
\Lambda_B:=\{y \in [0,1]^{\N} \; | \; y^{(j)} \in \Lambda_j, \; \forall j \in \N\}. \label{eq_bethe_cap}
\end{align}
From Section \ref{local_gibbs}, recall that $y^{(j)}=[y_k]_{k \in \N_j}$ is the local service rate vector, and $\Lambda_j$ defined in \eqref{eq_loc_cap} is the local capacity region which is nothing but the convex hull of the local feasible schedules $\I_j$.  In other words, a local service rate vector $y^{(j)}$ belongs to $\Lambda_j$, if and only if there exists a distribution $\b_j$ on the local feasible schedules $\I_j$, that supports the service rates $y^{(j)}$, \ie, $ y_k= \sum_{\{\x^{(j)} \in \I_j | x_k=1\}} \b_j(\x^{(j)}), \; \;  k \in \N_j$. As this definition of $\Lambda_B$ imposes only local feasibility of service rates, it is easy to argue that the Bethe capacity region is a relaxation of the actual capacity region, \ie, $\Lambda \subseteq \Lambda_B$.

%This definition is motivated from the concept of pseudo-marginals discussed in Section \ref{preliminaries_bethe}. Compared to a set of fully consistent marginals (\ie, a set of marginals for which there exists a coherent joint distribution), the pseudo-marginals have to satisfy only a relaxed set of constraints. Hence it follows that the actual capacity region is contained in the Bethe approximated capacity region, \ie, $\Lambda \subseteq \Lambda_B$.

Secondly, we scale the objective function  \eqref{eq_util_main} by a factor $\theta$, and add local entropy terms. The resulting new optimization problem is given by
\begin{align}
&\max_{y, \{\b_j\}}  \; \; \theta \;\sum_{j=1}^N U_j(y_j) + \sum_{j=1}^N H(\b_j), \; \; \; \; \text{subject to } \label{eq_util_bethe} \\
&y \in [0,1]^{\N}; \; \; \b_j(\x^{(j)}) \geq 0, \; \; \x^{(j)} \in \mathcal{I}_j, \; j=1 \dots N ; \; \nonumber\\
 &\sum_{\x^{(j)} \in \mathcal{I}_j} \b_j(\x^{(j)})=1,\; \;  j=1 \dots N; \nonumber \\
& \;  y_k= \sum_{\{\x^{(j)} \in \I_j | x_k=1\}} \b_j(\x^{(j)}), \; \;  k \in \N_j,\; j=1 \dots N . \label{eq_util_constraint}
\end{align}
Here, the constraint set is specified by explicitly expanding the definition of $\Lambda_j$ involved in description of $\Lambda_B$ \eqref{eq_bethe_cap}. For a large $\theta$, this new objective function \eqref{eq_util_bethe} closely approximates the original objective \eqref{eq_util_main} since the entropy is bounded from above and below. The advantage of defining this new optimization problem is that it is amenable to a distributed solution \cite{libin}. In particular, our local algorithm solves this problem in a distributed fashion.

\noindent  \emph{Step 2:} In the following Lemma, we show that Algorithm 2 solves the new optimization problem \eqref{eq_util_bethe}. 
\begin{lemma} \label{lemma_sub_grad}
Let $(\underline{s}, \{\underline{\b}_j\})$ be the solution of the optimization problem \eqref{eq_util_bethe}. Then the service rates $\{s_j(t)\}$ \eqref{eq_one_dim} in Algorithm 2 converge to the limit $\underline{s}=\{\underline{s}_j\}$.
\end{lemma}
%\begin{lemma}
%Consider $\underline{s} = \lim_{t \rightarrow \infty} s(t)$. Then the optimization problem \eqref{eq_util_bethe} attains its maximum at $(\underline{s}, \{\underline{\b}_j\})$ for some $\{\underline{\b}_j\}$.
%\end{lemma}
\begin{proof}
The outline of the proof is to show Algorithm 2 corresponds to the dual subgradient method for \eqref{eq_util_bethe}. The proof is provided in Appendix \ref{proof_sub_grad}. % of the supplementary material.
%Appendix \ref{proof_sub_grad}. 
\end{proof}

\noindent {Step 3:}
We now show that the solution of the optimization problem \eqref{eq_util_bethe} achieves the performance guarantee claimed in \eqref{eq_thm_util}. In other words, we show that $\underline{s}=\{\underline{s}_j\}$ satisfies \eqref{eq_thm_util}.

Recollect that we have added the local entropy terms to the actual objective function to obtain a new problem \eqref{eq_util_bethe}. Here, we shall evaluate the effect of these entropy terms on the optimal utility. To that end, let us consider $(\underline{s}, \{\underline{\b}_j\})$, the solution to the maximization problem \eqref{eq_util_bethe}.  Let us also consider the following optimization problem which does not have the local entropy terms. $s^*:= \arg \max_{y \in \Lambda_B} \sum_j U_j(y_j).$
Note that $s^*$ could be different from $\underline{s}$. Also, from the definition of $\Lambda_B$, for every $y \in \Lambda_B$ there exists some $\{\b_j\}$ such that $(y, \{\b_j\})$ is feasible for the problem \eqref{eq_util_bethe}. Hence for $s^* \in \Lambda_B$, there exists some $\{\b_j^*\}$ such that $(s^*, \{\b_j^*\})$ is feasible for \eqref{eq_util_bethe}. Then,
\begin{align}
\theta \sum_j U_j(s^*_j) &\leq \theta \sum_j U_j(s_j^*) + \sum_j H(\b^*_j), \nonumber\\
&\overset{(a)}{\leq} \theta \sum_j U_j(\underline{s}_j) + \sum_j H(\underline{\b}_j), \nonumber\\
&\overset{(b)}{\leq} \theta \sum_j U_j(\underline{s}_j) + \sum_j \log |\mathcal{I}_j|, \label{eq_entropy1}
\end{align}
where $(a)$ follows from the fact that $(\underline{s}, \{\underline{\b}_j\})$ maximizes \eqref{eq_util_bethe}, $(b)$ follows from the fact that entropy $H(\b_j) \leq \log |\mathcal{I}_j|$. Next, using the fact that $\Lambda \subseteq \Lambda_B$, we have
\begin{align}
\max_{y \in \Lambda} \sum_j U_j(y_j) &\leq \max_{y \in \Lambda_B} \sum_j U_j(y_j) = \sum_j U_j(s^*_j). \label{eq_entropy2}
\end{align}

\noindent Using \eqref{eq_entropy2} in \eqref{eq_entropy1} completes the proof of Theorem \ref{thm_util}.
%\end{proof}
\end{proof}

We conclude this section by contrasting our utility maximization algorithm with a prior work \cite{libin} which is also a subgradient descent based algorithm. The key difference between these works is in the complexity involved in computing the subgradients. Specifically, in our algorithm, the complexity of computing the subgradient is independent of the total size of the network. On the other hand, it could be exponentially large in the network size, for the algorithm given in \cite{libin}.

